Near Optimal Exploration-Exploitation in Non-Communicating Markov Decision Processes

While designing the state space of an MDP, it is common to include states that are transient or not reachable by any policy (e.g., in mountain car, the product space of speed and position contains configurations that are not physically reachable). This leads to defining weakly-communicating or multi-chain MDPs. In this paper, we introduce \tucrl, the first algorithm able to perform efficient exploration-exploitation in any finite Markov Decision Process (MDP) without requiring any form of prior knowledge. In particular, for any MDP with $S^{\texttt{C}}$ communicating states, $A$ actions and $\Gamma^{\texttt{C}} \leq S^{\texttt{C}}$ possible communicating next states, we derive a $\widetilde{O}(D^{\texttt{C}} \sqrt{\Gamma^{\texttt{C}} S^{\texttt{C}} AT})$ regret bound, where $D^{\texttt{C}}$ is the diameter (i.e., the longest shortest path) of the communicating part of the MDP. This is in contrast with optimistic algorithms (e.g., UCRL, Optimistic PSRL) that suffer linear regret in weakly-communicating MDPs, as well as posterior sampling or regularised algorithms (e.g., REGAL), which require prior knowledge on the bias span of the optimal policy to bias the exploration to achieve sub-linear regret. We also prove that in weakly-communicating MDPs, no algorithm can ever achieve a logarithmic growth of the regret without first suffering a linear regret for a number of steps that is exponential in the parameters of the MDP. Finally, we report numerical simulations supporting our theoretical findings and showing how TUCRL overcomes the limitations of the state-of-the-art.

==> app_regret.tex <==
% !TEX root = tucrl.tex

\section{Regret of \tucrl}\label{app:tucrl.regret}
\begin{algorithm}[t]
        \caption{\textsc{Truncated Extended Value Iteration (Tevi)}}
        \begin{algorithmic}
                \STATE\textbf{Input:} value vector $\wt{h}_0$, extended MDP $\mathcal{M}$, set of states $\wb{\calS}$, accuracy $\epsilon$
                \STATE\textbf{Output:} $\wt{g}_k$, $\wt{h}_k$, $\wt{\pi}_k$
                \STATE $k := 0$
                \STATE $\wt{h}_1(s) := \wt{L}_{\mathcal{M}} \wt{h}_0(s) := \max_{a \in \A_s} \left\{\max_{\wt{r} \in B_{r}(s,a)} \wt{r} +  \max_{\wt{p} \in B_{p}(s,a)} \wt{p}^\transp \wt{h}_0 \right\}$, $\forall s \in \wb{\calS}$ (see Sec.~\ref{sec:tucrl})
                \WHILE{$\max_{s\in \wb{\calS}} \left\{ \wt{h}_{k+1}(s) - \wt{h}_k(s) \right\} -  \min_{s\in \wb{\calS}} \left\{ \wt{h}_{k+1}(s) - \wt{h}_{k}(s) \right\} > \epsilon$}
                    \STATE $k := k + 1$
                    \STATE $\wt{h}_{k+1}(s) := \wt{L}_{\mathcal{M}} \wt{h}_{k}(s)$, $\forall s \in \wb{\calS}$
                \ENDWHILE
                \STATE $\wt{g}_k :=\frac{1}{2} \left(\max_{s\in \wb{\calS}} \left\{ \wt{h}_{k+1}(s) - \wt{h}_k(s) \right\} + \min_{s\in \wb{\calS}} \left\{ \wt{h}_{k+1}(s) - \wt{h}_{k}(s) \right\} \right)$
                \STATE $\wt{\pi}_k(s) \in \argmax_{a \in \A_s} \left\{\max_{\wt{r} \in B_{r}(s,a)} \wt{r} +  \max_{\wt{p} \in B_{p}(s,a)} \wt{p}^\transp \wt{h}_{k} \right\}$, $\forall s \in \wb{\calS}$
        \end{algorithmic}
        \label{alg:tevi}
\end{algorithm}


We follow the proof structure of~\citet{Jaksch10,fruit2018constrained} and use similar notations. Nonetheless, several parts of the proof significantly differ from \citep{Jaksch10,fruit2018constrained}:
\begin{itemize}
 \item in Sec.~\ref{app:regret.Minset} we prove that after a finite number of steps, \tucrl is \emph{gain-optimistic} (which is not as straightforward as in the case of \ucrl),
 \item in Sec.~\ref{sec:bound_wt_delta} we show that the sums taken over the whole state space $\calS$ that appear in the main term of the regret decomposition of \ucrl can be restricted to sums over $\calScom_k$ thanks to the new stopping condition used for episodes and the use of the condition $N_k^\pm(s,a) > \sqrt{\sfrac{t_k}{SA}}$ (see~\eqref{eqn:restricted_summation}),
 \item in Sec.~\ref{sec:poorly.visited.states}, we bound the number of time steps spent in ``bad''\todomout{poorly visited??} state-action pairs $(s,a)$ satisfying $N_k^\pm(s,a) \leq \sqrt{\sfrac{t_k}{SA}}$,
 \item in Sec.~\ref{app:regret.number.episodes}, we bound the number of episodes with the new stopping condition.
\end{itemize}



\subsection{Splitting into episodes}
The regret of \tucrl after $T$ time steps is defined as:
\[
        \Delta(\tucrl, T) := Tg^* - \sum_{t=1}^T r_t(s_t,a_t) 
\]
% Similarly to what is done with \ucrl \citep{Jaksch10}, we index the episodes of \tucrl by $k$.
% Episode $k$ starts at time $t_k$, and for any state-action pair $(s,a)$ we denote by $N_k(s,a)$ the number of visits in $(s,a)$ prior to episode $k$ ($k$ not included) and by $\nu_k(s,a)$ the number of visits in $(s,a)$ during episode $k$:
% \begin{align}\label{eqn:N_nu}
% \begin{split}
%  N_{k}(s,a) := \sum_{t=1}^{t_k-1}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace~~ &\text{and} ~~
%  \nu_k(s,a) := \sum_{t=t_k}^{t_{k+1}-1}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace\\
%  \implies N_{k}&(s,a) = \sum_{i=1}^{k-1}\nu_i(s,a)
%  \end{split}
% \end{align}
% By convention, we denote by $N_{k_T+1}(s,a):= \sum_{t=1}^{T}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace$ the total number of visits in $(s,a)$ up to time $T$ ($T$ included). We will also use the convenient notations $N_k^+(s,a):= \max\lbrace 1,N_k(s,a)\rbrace$ and $N_k^\pm(s,a):= \max\lbrace 1,N_k(s,a)-1\rbrace$ for the maximum value between $1$ and $N_k(s,a)$ or $N_k(s,a)-1$. This term will frequently appear in the proof. The stopping condition of episodes used by \tucrl implies that
% \begin{align}\label{eqn:stopping_condition_ineuality}
%  \forall k \geq 1, \forall (s,a) \in S \times A, ~~ \nu_{k}(s,a) \leq N_k^+(s,a)
% \end{align}
We denote by $k_t := \sup \lbrace k \geq 1:~~ t_k \leq t\rbrace$ the current episode at time $t$. The action played by \tucrl at time $t$ is $\wt{\pi}_{k_t}(s_t)$ and we can rewrite the regret as
\begin{align*}
  \Delta(\tucrl, T) = Tg^* - \sum_{t=1}^T r_t(s_t,\widetilde{\pi}_{k_t}(s_t))
\end{align*}
Let's define the filtration $\mathcal{F}_t = \sigma(s_1, a_1,r_1,\dots,s_{t+1})$ and the stochastic process $Y_t = r_t(s_t,\widetilde{\pi}_{k_t}(s_t)) - r(s_t,\widetilde{\pi}_{k_t}(s_t))$. Note that both $k_t$ and $\widetilde{\pi}_{k_t}(s_t)$ are $\mathcal{F}_{t-1}$-measurable. Moreover, $(Y_t,\mathcal{F}_t)_{t\geq 0}$ is a Martingale Difference Sequence (MDS) since $|Y_t| \leq \rmaxbound$ and $\mathbb{E}[Y_t | \mathcal{F}_{t-1}] = 0$. Using Azuma's inequality \citep[see \eg][Lemma 10]{Jaksch10}:
\begin{align*}
 \mathbb{P}\left(\sum_{t=1}^T r_t(s_t,\widetilde{\pi}_{k_t}(s_t)) \leq \sum_{t=1}^T r(s_t,\widetilde{\pi}_{k_t}(s_t)) - \rmaxbound\sqrt{\frac{5}{2}T\ln \left(\frac{8T}{\delta}\right)}\right) \leq \left(\frac{\delta}{8T}\right)^{5/4} < \frac{\delta}{12T^{5/4}}
\end{align*}
Defining $\Delta_k = \sum_{s\in\calS, a \in \A} \nu_k(s,a) \left( g^* - r(s,a) \right)$ it holds with probability $1 - \frac{\delta}{12T^{4/5}}$ that:
\begin{align}\label{eqn:martingale_reward}
\begin{split}
        \Delta(\tucrl, T) &\leq  Tg^* - \sum_{s,a} N(s,a) r(s,a) + \rmaxbound\sqrt{\frac{5}{2}T\ln \left(\frac{8T}{\delta}\right)}\\
                          &= \sum_{k=1}^{m} \sum_{s,a} \nu_k(s,a) g^* - \sum_{k=1}^{m} \sum_{s,a} \nu_k(s,a) r(s,a) +\rmaxbound\sqrt{\frac{5}{2}T\ln \left(\frac{8T}{\delta}\right)}\\
                          &= \sum_{k=1}^m \Delta_k + \rmaxbound\sqrt{\frac{5}{2}T\ln \left(\frac{8T}{\delta}\right)}
\end{split}
\end{align}

\subsection{Dealing with Failing Confidence Intervals ($M^* \notin \mathcal{M}_k$)}
We start by bounding the term $\sum_{k=1}^m \Delta_k \mathbbm{1}{\lbrace M^* \not\in \mathcal{M}_k \rbrace}$ corresponding to the regret suffered in episodes where the true MDP $M^*$ is not contained in the original set of plausible MDPs $\mathcal{M}^1_k$. 
We use exactly the same proof as in~\citep{Jaksch10,fruit2018constrained}.
Start noticing that the stopping condition of episodes used by \tucrl implies that (see Alg.~\ref{fig:ucrl.constrained}):
\begin{align}\label{eqn:stopping_condition_ineuality}
 \forall k \geq 1, ~\forall (s,a) \in \calS \times \A, ~~ \nu_{k}(s,a) \leq N_k^+(s,a)
\end{align}
Then, as is proved in Appendix F.2 of \citep{fruit2018constrained}, since both \eqref{eqn:stopping_condition_ineuality} and Theorem 1 of \citet{fruit2018constrained} hold, we have that with probability at least $1-\frac{\delta}{20T^{5/4}} \geq 1-\frac{\delta}{12T^{5/4}}$:
\begin{align}\label{eqn:failed_episodes}
 \sum_{k=1}^m \Delta_k \mathbbm{1}{\lbrace M^* \not\in \mathcal{M}_k \rbrace} \leq {\rmaxbound} \sqrt{T}
\end{align}

\subsection{Episodes with $M^* \in \mathcal{M}_k$}\label{app:regret.Minset}
We now assume that $M^* \in \mathcal{M}_k$. Let's denote by $\wt{g}_k$, $\wt{h}_k$ and $\wt{\pi}_k$ the outputs of $\tevi(\bm{0}, \mathcal{M}_k^\diamond, \calS_k, \varepsilon_k)$ (see Alg.~\ref{alg:tevi}) where $\varepsilon_k := \rmaxbound/\sqrt{t_k}$ and
\begin{equation}
         \label{eq:tucrl.optimization}
%         (\wt{M}_k, \wt{\pi}_k) = \argmax_{M \in \mathcal{M}_k^\diamond, \pi \in \Pi^{\textsc{SD}}(M)} \{g^{\pi}_M\}
        \calS_k = \begin{cases}
                \calScom_k & \text{if } \mathcal{K}_k = \emptyset \\
                \calS & \text{otherwise}
        \end{cases},
%         \qquad \text{where } 
        ~~ \mathcal{M}_k^\diamond = \begin{cases}
                \mathcal{M}_k=\wb{\mathcal{M}}_k & \text{if } \calStrans_k = \emptyset\\
                \wb{\mathcal{M}}_k^{+} & \text{otherwise}
        \end{cases}.
\end{equation}
In order to bound $\Delta_k$ we first show that $\wt{g}_k \gtrsim g^*$ (up to $\rmaxbound/\sqrt{t_k}$-accuracy). If $\calStrans_k = \emptyset$ then by definition 
% $\mathcal{M}_k^{2+} = \mathcal{M}_k^{1+}$ implying $M^*  \in \mathcal{M}^1_k \subseteq \mathcal{M}^{1+}_k = \mathcal{M}_k^{2+}$
$\mathcal{M}_k^{\diamond} = \wb{\mathcal{M}}_k = \mathcal{M}_k \ni M^*$
and so we can use the same argument as in~\citep[][Sec. 4.3 \& Thm. 7]{Jaksch10}. If  $\calStrans_k \neq \emptyset$, the true MDP $M^*$ might not be ``included'' in the extended MDP $\wb{\mathcal{M}}_k^{+}$ considered by \evi and we cannot use the same argument. 
To overcome this problem we split the analysis based on the level of exploration achieved so far.

\paragraph{Poorly explored episodes:} we first consider the case 
\begin{equation}\label{eqn:def_f}
        t_k < \frac{2401}{9}\Big(\diamcom\Big)^2SA \cdot\left(\Strans_k \ln\left(\frac{2SAt_k}{\delta}\right)\right)^2 := C(k)
\end{equation}
where $\Strans_k:= \left| \calStrans_k \right|$ is the cardinal of $\calStrans_k$.
By definition for all $ k \geq 1$, \[\Delta_k = \sum_{t=t_k}^{t_{k+1}-1}\left(g^*-r(s_t,a_t)\right) \leq \rmaxbound(t_{k+1}-t_k)\] and as a consequence of \eqref{eqn:stopping_condition_ineuality} \[t_{k+1} = t_k + \sum_{s,a}\underbrace{\nu_k(s,a)}_{\leq N_k(s,a)} \leq  t_k+\sum_{s,a}N_k(s,a) = 2t_k \]
Defining $k^* = \max \left\lbrace k \geq 1 : ~ t_k < C(k) \right\rbrace$ we have
\begin{align}
 \sum_{k=1}^{m}\Delta_k\cdot\underbrace{\mathbbm{1}\lbrace t_k < C(k) \rbrace}_{\geq 0} &\leq \rmaxbound \sum_{k=1}^{m}(t_{k+1}-t_k)\cdot\mathbbm{1}\lbrace t_k < C(k) \rbrace \nonumber \\
 &= \rmaxbound \sum_{k=1}^{k^*}(t_{k+1}-t_k) = \rmaxbound ( t_{k^*+1} -1) \leq 2\rmaxbound t_{k^*} \nonumber\\
 &\overset{(a)}{\leq}  2 \rmaxbound C(k) \nonumber \\ %~~ \text{by definition of }~k^* \nonumber\\
 & \leq \frac{4802}{9} \rmaxbound \Big(\diamcom\Big)^2S^3A  \ln^2\left(\frac{2SAT}{\delta}\right) \label{eqn:regret_bound_first_episodes}
\end{align}
where $(a)$ follows from the definition of $k^*$.

\paragraph{Sufficiently explored episodes:} from now on we will assume that the reverse inequality holds \ie
\begin{equation}\label{eq:tkbig}
        t_k \geq \frac{2401}{9}\Big(\diamcom\Big)^2SA\left(\Strans_k \ln\left(\frac{2SAt_k}{\delta}\right)\right)^2
\end{equation}
We now prove a useful lemma.
\begin{lemma} \label{L:M.com}
        Let episode $k$ be such that $M^* \in \mathcal{M}_k$, $\calStrans_k\neq \emptyset$ and ~\eqref{eq:tkbig} holds. Then,
        \[
                \left( \forall (s,a) \in \calScom_k \times \A, N_k^\pm(s,a) > \sqrt{\frac{t_k}{SA}} \right) \implies \calStrans_k = \calStrans
        \]
\end{lemma}
\begin{proof}       
        Assume that episode $k$ is such that~\eqref{eq:tkbig} holds 
%        $t_k \geq \Big(\diamcom\Big)^2SA\left(\Strans_k\right)^2 \ln\left(\frac{t_kSA}{\delta}\right)$
        and that for any state-action pair $(s,a) \in \calScom_k\times \A$
        \[
                N_k^\pm(s,a) > \sqrt{\frac{t_k}{SA}} \geq \frac{49}{3} \diamcom\Strans_k \ln\left(\frac{2SAt_k}{\delta}\right)
        \]
        Since $\calStrans_k\neq \emptyset$ and $M^* \in \mathcal{M}_k$, for any $(s,a,s') \in \calScom_k \times \A \times \calStrans_k$
        \begin{align*}
                \underbrace{p(s'|s,a)}_{\text{transition probability in }M^*} &\leq \underbrace{\wh{p}_k(s'|s,a)}_{=0} + \beta_k^{sas'} = \underbrace{\sqrt{\frac{14 \wh{\sigma}_{p,k}^2(s'|s,a) \ln(2 SA t_k/\delta)}{N_k^+(s,a)}}}_{=0} +\frac{49 \ln(2 SA t_k/\delta)}{3 N_k^\pm(s,a)}\\ &\leq \frac{49\ln\left(2SAt_k/\delta\right)}{3N_k^\pm(s,a)}
                < \frac{1}{\diamcom \Strans_k} 
        \end{align*}
        where we have exploited the fact that $\wh{p}(s'|s,a) =0$ and $\wh{\sigma}_{p,k}^2(s'|s,a) = 0$ for any state $s'\in\calStrans_k$ (remember that $N_k(s,a,s') =0$).

        We denote by $\tau_{M^*}(s \to s')$ the shortest path between any pair of states $(s,s') \in \calS \times \calS$ in the true MDP $M^*$.
        Fix an arbitrary target state $\wb{s} \in \calStrans_k$ and denote by $\tau(s) := \tau_{M^*}(s \to \wb{s})$ and $\tau_{\min}:= \min_{s \in \calScom_k}\{ \tau(s)\}$. We have
        \begin{align*}
                \tau(\wb{s}) &= 0\\
                \forall s \in \calScom_k \quad 
                \tau(s) &= 1+ \min_{a\in\A_s} \left \{\sum_{s'\in\calS} \underbrace{p(s'|s,a) \tau(s')}_{\geq 0} \right\}
                \geq 1+ \min_{a\in\A_s} \left \{\sum_{s'\in\calScom_k} p(s'|s,a) \underbrace{\tau(s')}_{\geq \tau_{\min}} \right\}\\ 
                &\geq 1 + \tau_{\min} \cdot \min_{a\in\A} \left\{ \sum_{s' \in \calScom_k} p(s'|s,a) \right\}
                 = 1 + \tau_{\min} \cdot\min_{a\in\A} \left\{  1 - \sum_{s' \in \calStrans_k} \underbrace{p(s'|s,a)}_{< {\frac{1}{\diamcom \Strans_k}}}  \right\}\\
                & > 1 + \tau_{\min} \left( 1 - \sum_{s' \in \calStrans_k} \frac{1}{\diamcom \Strans_k} \right) = 1 + \tau_{\min} \left( 1 - \frac{1}{\diamcom } \right)
        \end{align*}
        Applying the above inequality to $\wt{s} \in \calScom_k$ achieving $\tau(\wt{s}) = \tau_{\min}$ yields $\tau_{\min} > \diamcom$.
        This implies that the shortest path in $M^*$ between any state $s \in \calScom_k \subseteq \calScom$ and any state in $\wb{s} \in \calStrans_k$ is strictly bigger than $\diamcom$ but by definition $\diamcom$ is the longest shortest path between any pair of states in $\calScom$. Therefore, $\wb{s} \in \calStrans$.
%         it means that $\wb{s} \notin \calScom$ since $\tau_{\min}$ is bigger than the diameter of the communicating part of $M$.
        Since $\wb{s} \in \calStrans_k$ was chosen arbitrarily, then $\calStrans_k = \calStrans$.
\end{proof}
As a consequence of Lem.~\ref{L:M.com}, under the assumptions that $M^* \in \mathcal{M}_k$, $\calStrans_k\neq \emptyset$ and ~\eqref{eq:tkbig} holds, there are only two possible cases:
\begin{enumerate}
        \item Either $\calStrans_k = \calStrans$,
        \item or $\exists (s,a) \in \calScom_k \times \A \;:\; N_k^\pm(s,a) \leq \sqrt{\frac{t_k}{SA}}$.
\end{enumerate}

\textbf{Case 1:} $\calStrans_k = \calStrans$ implies that $M^* \in \wb{\mathcal{M}}_k^{+}$.
This is because for any $(s,a,s') \in \calScom_k \times \A \times \calStrans_k$ we have $p(s'|s,a) = \wt{p}_k(s'|s,a) =  0$ and for any $(s,a,s') \notin \calScom_k \times \A \times \calStrans_k$ we have  $p(s'|s,a) \in B_{p,k}(s,a,s') = \wb{B}_{p,k}(s,a,s') $ and so $p(\cdot|s,a) \in \wb{B}_{p,k}^{+}(s,a)$ {\color{red} TODO: write a ``proposition'' stating this result formally outside the regret proof}.
% Note that \tucrl is applying extended value iteration to $\mathcal{M}_k^{2+}$ where $B_{p,k}^{2+}(s,a) = \sum_{s'} B_{p,k}^2 (s,a,s')$:
% \begin{equation*}
%         (\wt{M}_k, \wt{\pi}_k) = \argmax_{M \in \mathcal{M}_k^{2+}, \pi \in \Pi^{\textsc{SD}}(M)} \{g^{\pi}_M\}
% \end{equation*}
Since $M^* \in \wb{\mathcal{M}}_k^{+}$, we can use the same argument as \citet[Sec. 4.3 \& Theorem 7]{Jaksch10} to prove $\wt{g}_k \geq g^* - \frac{\rmaxbound}{\sqrt{t_k}}$.

\textbf{Case 2:} For any $(s,a) \in \calStrans_k \times \A $, 
% $B_{p,k}^{2+}(s,a) = \{ (p(s))_{s\in \calS}: \sum_s p(s) = 1~\text{and}~p(s) \geq 0,~ \forall s \in \calS \}$ which is the set of all possible transition probabilities
$\wb{B}_{p,k}^{+}(s,a) = \mathcal{C}$
is the $(S-1)$-simplex denoting the maximal uncertainty about the transition probabilities, and $B_{r,k}(s,a) =[0, \rmaxbound]$.
We will now construct an MDP $M' \in \wb{\mathcal{M}}_k^{+}$ with optimal gain $\rmaxbound$.
For all $(s,a) \in \calStrans_k \times \A $, we set the transitions to $p_{M'}(s|s,a) = 1$ and rewards to $r_{M'}(s,a) = \rmaxbound$.
Let $(\wb{s},\wb{a})\in \calScom_k \times \A$ such that $N_k^\pm(\wb{s},\wb{a}) \leq \sqrt{\frac{t_k}{SA}}$ (which exists by assumption).
We set $p_{M'}(s'|\wb{s},\wb{a}) >0$ for all $s' \in \calStrans_k$. This is possible because by definition of $\wb{\mathcal{M}}_k^{+}$, the support of $p(\cdot|\wb{s},\wb{a})$ is not restricted to $\calScom_k$.
Finally, for all state-action pairs $(s,a) \in \calScom_k \times \A $, we set $p_{M'}(\wb{s}|s,a) >0$.
This is possible because by definition of $\wb{\mathcal{M}}_k^{+}$, the support of $p(\cdot|s,a)$ is only restricted to $\calScom_k$ and $\wb{s} \in \calScom_k$.
In $M'$, for all policies, all states in $\calStrans_k$ are absorbing states (\ie loop on themselves with probability 1) with maximal reward $\rmaxbound$ and all other states $s \in \calScom_k$ are transient.
The optimal gain of $M'$ is thus $\rmaxbound$ and since $M' \in \wb{\mathcal{M}}_k^{+}$ we conclude that $\wt{g}_k \geq \rmaxbound - \frac{\rmaxbound}{\sqrt{t_k}} \geq g^* - \frac{\rmaxbound}{\sqrt{t_k}}$.
% Then EVI in $\mathcal{M}_k^{2+}$ selects an mdp $\wt{M}_k$ and a policy $\wt{\pi}_k$ such that $\wt{p}_{\wt{M}_k}(s|s,a) = 1$ and $\wt{r}_{\wt{M}_k}(s,a) = \rmaxbound$ for any $(s,a) \in \calStrans_k \times \A$. As a consequence, for any $s \in \calStrans_k$, $g^{\wt{\pi}_k}_{\wt{M}_k}(s) = \rmaxbound$ but since $\calStrans_k$ is reachable from $\calScom_k$ and EVI recovers a policy with constant gain~\citep[see][]{Jaksch10} $\wt{g}_k \geq \rmaxbound - \frac{\rmaxbound}{\sqrt{t_k}} \geq g^* - \frac{\rmaxbound}{\sqrt{t_k}}$.

In conclusion, \evi is always returning an \emph{optimistic} policy when the assumptions of Lem.~\ref{L:M.com} hold. The regret $\Delta_k$ accumulated in episode $k$ can thus be upper-bounded as:
\begin{align*}
\Delta_k &=  \sum_{s,a}\nu_k(s,a)(g^* - r(s,a))  =  \sum_{s,a}\nu_k(s,a)(\underbrace{g^*}_{\mathclap{\leq \wt{g}_k - \frac{\rmaxbound}{\sqrt{t_k}}}} -\wt{r}_k(s,a)) 
+  \sum_{s,a}\nu_k(s,a)(\wt{r}_k(s,a) - r(s,a))\\ & \leq \underbrace{\sum_{s,a}\nu_k(s,a)(\wt{g}_k -\wt{r}_k(s,a))}_{:=\wt{\Delta}_k} +  \sum_{s,a}\nu_k(s,a)(\wt{r}_k(s,a) - r(s,a)) + \rmaxbound \sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}}\end{align*}
To bound the difference between the optimistic reward $\wt{r}_k$ and the true reward $r$ we introduce the estimated reward $\wh{r}_k$:
\begin{align*}
 \forall s,a \in \calS \times \mathcal{A}, ~~\wt{r}_k(s,a) - r(s,a) = \underbrace{\wt{r}_k(s,a) -\wh{r}_k(s,a)}_{\leq \beta_{r,k}^{sa} ~\text{by construction}} + \underbrace{\wh{r}_k(s,a) - r(s,a)}_{\leq \beta_{r,k}^{sa} ~ \text{since} ~ M \in \mathcal{M}_k} \leq 2 \beta_{r,k}^{sa}
\end{align*}
and so in conclusion:
\begin{align}\label{eqn:regret_bound_decomposition_1}
\Delta_k \leq \wt{\Delta}_k + 2\sum_{s,a}\nu_k(s,a) \beta_{r,k}^{sa} + \rmaxbound \sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}}
\end{align}

\subsection{Bounding $\wt{\Delta}_k$}\label{sec:bound_wt_delta}

The goal of this section is to bound the term \[\wt{\Delta}_k := \sum_{s,a}\nu_k(s,a)(\wt{g}_k -\wt{r}_k(s,a)) = \sum_{s}\nu_k(s,\wt{\pi}_k(s))(\wt{g}_k -\wt{r}_k(s,\wt{\pi}_k(s)))\]

We start by discarding the state-action pairs $(s,a)$ that have been poorly visited so far \ie satisfying $N_k^\pm(s,a) \leq \sqrt{\frac{t_k}{SA}}$:
\begin{align}
 \wt{\Delta}_k &= \sum_{s,a}\nu_k(s,a)(\wt{g}_k -\wt{r}_k(s,a)) \nonumber\\
 &= \sum_{s,a}\nu_k(s,a)(\wt{g}_k -\wt{r}_k(s,a))\underbrace{\mathbbm{1}\lbrace N_k^\pm(s,a)>\sqrt{\sfrac{t_k}{SA}} \rbrace}_{:= \mathbbm{1}_{k}(s,a)}\nonumber\\ 
 &\quad{} + \sum_{s,a}\nu_k(s,a)\underbrace{(\wt{g}_k -\wt{r}_k(s,a))}_{\leq \rmaxbound}\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{SA}} \rbrace \nonumber\\
 %\begin{split}
 &\leq \underbrace{\sum_{s,a}\nu_k(s,a)(\wt{g}_k -\wt{r}_k(s,a))\mathbbm{1}_{k}(s,a)}_{\wt{\Delta}'_k}
 + \rmaxbound \sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace 
 \label{eqn:wt_delta_bound_decomposition_1}
 %\end{split}
\end{align}
We will now bound the term 
\begin{align*}
\wt{\Delta}_k' :=\sum_{s,a}\nu_k(s,a)(\wt{g}_k -\wt{r}_k(s,a))\mathbbm{1}_{k}(s,a) = \sum_{s}\nu_k(s,\wt{\pi}_k(s))(\wt{g}_k -\wt{r}_k(s,\wt{\pi}_k(s)))\mathbbm{1}_{k}(s,\wt{\pi}_k(s))
\end{align*}
The policy $\wt{\pi}_k$ is obtained by executing $\tevi(0,\mathcal{M}_k^\diamond,\calS_k,\varepsilon_k)$~\ref{alg:tevi} where $\varepsilon_k:= \rmaxbound/\sqrt{t_k}$ and $\calS_k$ and $\mathcal{M}_k^\diamond$ are defined in~\eqref{eq:tucrl.optimization}.
In all possible cases for both $\calS_k$ and $\mathcal{M}_k^\diamond$, this amounts to applying value iteration to a \emph{communicating} MDP with finite state space $\calS_k$ and \emph{compact} action space.
By~\citep[Thm. 8.5.6]{puterman1994markov}, since the convergence criterion of value iteration is met we have:
\begin{align*}
 \forall s \in \calS_k, ~~\left|  \wt{h}_k(s) + \wt{g}_k - \wt{r}_k(s,\wt{\pi}_k(s)) - \sum_{s'\in \mathcal{S}} \wt{p}_k(s'|s,\wt{\pi}_k(s)) \wt{h}_k(s') \right| \leq \frac{\rmaxbound }{\sqrt{t_k}}
\end{align*}
For all $s \notin \calScom_k$, $\nu_k(s,\wt{\pi}_k(s)) =0$ due to the stopping condition of episode $k$. Therefore we can write:
\begin{align}\label{eqn:wt_delta_bound_decomposition_2}
\begin{split}
 \wt{\Delta}_k' 
 &\leq \sum_{s}\nu_k(s,\wt{\pi}_k(s))\left( \sum_{s'\in \mathcal{S}} \wt{p}_k(s'|s,\wt{\pi}_k(s)) \wt{h}_k(s') - \wt{h}_k(s) + \frac{\rmaxbound}{\sqrt{t_k}} \right)\mathbbm{1}_{k}(s,\wt{\pi}_k(s))\\
 &= \nu_k' \left( \wt{P}_k -I \right) \wt{h}_k + \rmaxbound \sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}}\mathbbm{1}_{k}(s,a)
 \end{split}
\end{align}
where $\nu_k' = (\nu_k(s,\wt{\pi}_k(s))\mathbbm{1}_{k}(s,\wt{\pi}_k(s)))_{s\in \calS}$ is the vector of visit counts for each state and the corresponding action chosen by $\wt{\pi}_k$ multiplied by the indicator function $\mathbbm{1}_{k}$, $\wt{P}_k = (\wt{P}_k(s'|s,\wt{\pi}_k(s)))_{s,s'\in\calS}$ is transition matrix associated to $\wt{\pi}_k$ in $\wb{\mathcal{M}}_k^{+}$ and $I$ is the identity matrix. We now focus on the term $\nu_k'(\wt{P}_k -I)\wt{h}_k$. Since the rows of $\wt{P}_k$ sum to 1, we have:
\begin{align*}
 \forall \lambda \in \Re, ~~ \left( \wt{P}_k -I \right) \wt{h}_k = \left( \wt{P}_k -I \right) \left( \wt{h}_k+\lambda e \right)
\end{align*}
where $e = (1,\dots 1)^\intercal$ is the vector of all ones. Let's take $\lambda := -\min_{s\in \calScom_k}{\lbrace \wt{h}_k(s) \rbrace}$ and define $w_k := \wt{h}_k +\lambda e$ so that for all $s\in \calScom_k$, $w_k(s)\geq 0$ and $\min_{s\in \calScom_k}{\lbrace w_k(s)\rbrace} =0$. We have:
% \begin{align*}
%  \nu_k'(\wt{P}_k -I)\wt{h}_k = \nu_k'(\wt{P}_k -I)w_k = \nu_k'(\wt{P}_k -P_k)w_k + \nu_k'(P_k - I)w_k
% \end{align*}
% We start by bounding $\nu_k'(\wt{P}_k -P_k)w_k$:
\begin{align*}
        \nu_k'(\wt{P}_k -I)\wt{h}_k &= \sum_{s\in \calS} \nu_k(s,\wt{\pi}_k(s))\mathbbm{1}_{k}(s,\wt{\pi}_k(s)) \left(\sum_{s'\in \calS}\wt{p}_k(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s) \right)
\end{align*}
Whenever $s_t \in \calStrans_{k_t}$, episode $k_t$ stops before executing any action (see the stopping condition of \tucrl in Alg.~\ref{fig:ucrl.constrained}) implying that $\forall s \in \calStrans_k$, $\nu_k(s,\wt{\pi}_k(s)) = 0$. Therefore we have:
\begin{align*}
        \nu_k'(\wt{P}_k -I)\wt{h}_k &= \sum_{s\in \calScom_k} \nu_k(s,\wt{\pi}_k(s))\mathbbm{1}_{k}(s,\wt{\pi}_k(s)) \left(\sum_{s'\in \calS}\wt{p}_k(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s) \right)
\end{align*}
For all states $s$ such that $\mathbbm{1}_{k}(s,\wt{\pi}_k(s))=1$ \ie satisfying $N_k^\pm(s,\wt{\pi}_k(s))>\sqrt{\sfrac{t_k}{SA}}$, we force \tevi to set $\wt{p}_k(s'|s,\wt{\pi}_k(s)) =0$, $\forall s' \in \calStrans_k$, by construction of $\wb{\mathcal{M}}_k^{+}$ so that:
% the difference $\wt{p}_k(s'|s,\wt{\pi}_k(s)) - p(s'|s,\wt{\pi}_k(s)$ is negative and $w_k(s') \geq 0$ by definition implying that
% $
%  \left(\wt{p}_k(s'|s,\wt{\pi}_k(s)) - p(s'|s,\wt{\pi}_k(s)) \right)w_k(s') \leq 0.
% $
\begin{align}\label{eqn:restricted_summation}
        \nu_k'(\wt{P}_k -I)\wt{h}_k = \sum_{s\in \calScom_k} \nu_k(s,\wt{\pi}_k(s))\mathbbm{1}_{k}(s,\wt{\pi}_k(s)) \left(\sum_{s'\in \calScom_k}\wt{p}_k(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s) \right)
\end{align}
We can now introduce $p$:
\begin{align}
 \notag
 \sum_{s'\in \calScom_k}
 \wt{p}_k(s'|s,\wt{\pi}_k(s))&w_k(s') - w_k(s)\\
 &= \sum_{s'\in \calScom_k} \wt{p}_k(s'|s,\wt{\pi}_k(s))w_k(s') - p(s'|s,\wt{\pi}_k(s))w_k(s') \label{eqn:wt_p_minus_p}\\ 
 &\quad{} + \left(\sum_{s'\in \calScom_k}p(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s) \right)\label{eqn:p_minus_identity}
\end{align}
The term \eqref{eqn:wt_p_minus_p} can be bounded as follows:
\begin{align*}
 \sum_{s'\in \calScom_k}\left(\wt{p}_k(s'|s,\wt{\pi}_k(s)) - p(s'|s,\wt{\pi}_k(s)) \right)w_k(s')
 &\leq \sum_{s'\in \calScom_k}\left|\wt{p}_k(s'|s,\wt{\pi}_k(s)) - p(s'|s,\wt{\pi}_k(s)) \right| w_k(s')\\
 &\leq \left\|\wt{p}_k(\cdot|s,\wt{\pi}_k(s)) - p(\cdot|s,\wt{\pi}_k(s)) \right\|_{1, \calScom} \max_{s' \in \calScom_k} \lbrace w_k(s')\rbrace
\end{align*}
where for any vector $v\in\Re^\calS$, $\|v\|_{1,\calScom}:=\sum_{s \in \calScom}|v(s)|$.

% \todom{
% The notation $\|\cdot\|_{1,\calScom}$ denotes the $\ell_1$-norm restricted on the states in $\calScom$.
% }
% In order to bound $\max_{s' \in \calScom_k} \lbrace w_k(s')\rbrace$ we first prove a lemma.
% \begin{lemma}\label{lem:minimum_span_S_k_1}
%  There exists a state $\wt{s}$ achieving the minimum value of $w_k$ \ie satisfying $w_k(\wt{s}) =\min_{s\in\calS}{\lbrace w_k(s) \rbrace}$, that belongs to $\calScom_k$ \ie $\wt{s}\in \calScom_k$.
% \end{lemma}
% \begin{proof}
%  Let $s \in \calStrans_k$. By definition of $\calStrans_k$, for any $a\in \mathcal{A}_s$, $N_k(s,a) =0$ implying that $B_p^k(s,a) = [0,1]$. Therefore, in $\mathcal{M}_k^{2+}$ 
% \end{proof}
Define $\overline{s} \in \argmax_{s\in\calScom_k}{\lbrace w_k(s) \rbrace}$ and $\wt{s} \in \argmin_{s\in\calScom_k}{\lbrace w_k(s) \rbrace}$.
By definition $\overline{s}, \wt{s} \in \calScom_k$ and $w_k(\wt{s})= \min_{s\in\calScom_k}{\lbrace w_k(s) \rbrace} =0$.
By Lem.~\ref{lem:span_shortest_path}, we know that for all $s,s'\in \calScom_k $,  the difference $w_k(s') - w_k(s) = \wt{h}_k(s') - \wt{h}_k(s)$ is upper bounded by $\rmaxbound \cdot\tau_{\wb{\mathcal{M}}_k^{+}}(s \rightarrow s')$.
We also know by Lem.~\ref{lem:same_shortest_path} that for all $s,s'\in \calScom_k,~\tau_{\mathcal{M}_k^{+}}(s \rightarrow s') =  \tau_{\wb{\mathcal{M}}_k^{+}}(s \rightarrow s')$. 
Since $M^*\in \mathcal{M}_k^{+}$ ($M^*$ is the true MDP), we also have that for all $s,s'\in \calScom_k,~\tau_{\mathcal{M}_k^{+}}(s \rightarrow s') \leq \tau_{M^*}(s \rightarrow s') \leq \diamcom$. In conclusion, 
 \begin{align}\label{eqn:span_bounded_diameter}
 \forall s,s'\in \calScom_k,~~w_k(s') - w_k(s)\leq \rmaxbound \diamcom
\end{align}
 and in particular
\begin{align*}
 \max_{s' \in \calScom_k} \lbrace w_k(s')\rbrace = w_k(\overline{s}) = w_k(\overline{s}) - \underbrace{w_k(\wt{s})}_{=0} \leq \rmaxbound \diamcom.
\end{align*}
To bound the distance in $\ell_1$-norm between $\wt{p}_k$ and $p$ we introduce $\wh{p}_k$:
\begin{align}
        \left\|\wt{p}_k(\cdot|s,\wt{\pi}_k(s)) - p(\cdot|s,\wt{\pi}_k(s)) \right\|_{1,\calScom}
        &\leq \underbrace{\left\|\wt{p}_k(\cdot|s,\wt{\pi}_k(s)) - \wh{p}_k(\cdot|s,\wt{\pi}_k(s)) \right\|_{1,\calScom}}_{\leq \sum_{s' \in \calScom} \beta_{p,k}^{s\wt{\pi}_k(s)s'} ~\text{by construction}} \nonumber\\
        &\quad{}+ \underbrace{\left\|\wh{p}_k(\cdot|s,\wt{\pi}_k(s)) - p(\cdot|s,\wt{\pi}_k(s)) \right\|_{1,\calScom}}_{= \sum_{s'\in \calScom}\left|\wh{p}_k(s'|s,\wt{\pi}_k(s)) - p(s'|s,\wt{\pi}_k(s))\right|}\nonumber\\
        &\leq  \sum_{s' \in \calScom} \beta_{p,k}^{s\wt{\pi}_k(s)s'} + \sum_{s'\in \calScom}\underbrace{\left|\wh{p}_k(s'|s,\wt{\pi}_k(s)) - p(s'|s,\wt{\pi}_k(s))\right|}_{\leq \beta_{p,k}^{s\wt{\pi}_k(s)s'} ~ \text{since} ~ M^* \in \mathcal{M}_k} \nonumber\\
        &\leq 2 \left(\sum_{s' \in \calScom} \beta_{p,k}^{s\wt{\pi}_k(s)s'} \right) \label{eqn:wt_delta_bound_decomposition_3}
\end{align}

We now bound the overall contribution of the term~\eqref{eqn:p_minus_identity}. \citet{Jaksch10} decompose this term into a martingale difference sequence and a telescopic sum but due to the indicator function $\mathbbm{1}_k$, in our case the sum is not telescopic anymore and an additional term appears.
\begin{align}
 \sum_{s\in \calScom_k} &\nu_k(s,\wt{\pi}_k(s))\mathbbm{1}_{k}(s,\wt{\pi}_k(s))\left(\sum_{s'\in \calScom_k}p(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s)\right)\nonumber\\
 &= \sum_{s\in \calS} \nu_k(s,\wt{\pi}_k(s))\mathbbm{1}_{k}(s,\wt{\pi}_k(s))\left(\sum_{s'\in \calScom_k}\underbrace{p(s'|s,\wt{\pi}_k(s))w_k(s')}_{\geq 0,~~ \forall s' \in \calScom_k}\mathbbm{1}{\lbrace s \in \calScom_k\rbrace} - w_k(s)\mathbbm{1}{\lbrace s \in \calScom_k\rbrace}\right)\nonumber\\
 &\leq \sum_{s\in \calS} \nu_k(s,\wt{\pi}_k(s))\mathbbm{1}_{k}(s,\wt{\pi}_k(s))\left(\sum_{s'\in \calScom_k}p(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s)\mathbbm{1}{\lbrace s \in \calScom_k\rbrace}\right)\nonumber\\
 &= \sum_{t=t_k}^{t_{k+1}-1} \left(\sum_{s'\in \calS_{k}^1}p(s'|s_t,\wt{\pi}_{k}(s_t))w_{k}(s')  - w_{k}(s_t)\mathbbm{1}{\lbrace s_t \in \calScom_k\rbrace} \right) \mathbbm{1}_{{k}}(s_t,\wt{\pi}_{k}(s_t))\nonumber\\
 &= \sum_{t=t_k}^{t_{k+1}-1} \underbrace{\left(\sum_{s'\in \calS_{k}^1}p(s'|s_{t},\wt{\pi}_{k}(s_{t}))w_{k}(s') - w_k(s_{t+1})\mathbbm{1}{\lbrace s_{t+1} \in \calScom_k\rbrace}\right) \mathbbm{1}_{k}(s_t,\wt{\pi}_k(s_t))}_{:=X_t} \label{eqn:mds}\\
 &\quad{}+ \underbrace{\sum_{t=t_k}^{t_{k+1}-1} \left(w_k(s_{t+1})\mathbbm{1}{\lbrace s_{t+1} \in \calScom_k\rbrace} - w_k(s_t)\mathbbm{1}{\lbrace s_{t} \in \calScom_k\rbrace} \right) \mathbbm{1}_{k}(s_t,\wt{\pi}_k(s_t))}_{\text{not telescopic due to }\mathbbm{1}_k!}\label{eqn:sum_not_telescopic}
\end{align}
Define the filtration $\mathcal{F}_{t} = \sigma(s_1,a_1, r_1,\dots, s_{t+1})$. Since $k_t$ is $\mathcal{F}_{t-1}$-measurable: 
\begin{align*}
 \mathbbm{E}\left[w_{k_t}(s_{t+1})\mathbbm{1}{\lbrace s_{t+1} \in \calScom_{k_t}\rbrace}\mathbbm{1}_{k_t}(s_t,\wt{\pi}_{k_t}(s_t))|\mathcal{F}_{t-1}\right] &= \underbrace{\sum_{s'\in \calScom_{k_t}}p(s'|s_{t},\wt{\pi}_{k_t}(s_{t}))w_{k_t}(s')\mathbbm{1}_{k_t}(s_t,\wt{\pi}_{k_t}(s_t))}_{\mathcal{F}_{t-1}-\text{measurable}}\\
 \implies \mathbbm{E}[X_{t}|\mathcal{F}_{t-1}]&=0
\end{align*}
and so $(X_t,\mathcal{F}_t)_{t\geq 1}$ is a martingale difference sequence (MDS) and $|X_t| \leq \rmaxbound \diamcom$. We will bound~\eqref{eqn:mds} in the next section (Sec.~\ref{sec:regret_bound_sum}) using Azuma's inequality.
Using the fact that $\mathbbm{1}_{k}(s_t,\wt{\pi}_k(s_t)) = 1 - \mathbbm{1}\lbrace N_k^\pm(s_t,\wt{\pi}_k(s_t))\leq\sqrt{\sfrac{t_k}{SA}}\rbrace$ we can make a telescopic sum appear and rewrite \eqref{eqn:sum_not_telescopic} as:
\begin{align}
 \sum_{t=t_k}^{t_{k+1}-1} &\left(w_k(s_{t+1})\mathbbm{1}{\lbrace s_{t+1} \in \calScom_k\rbrace} - w_k(s_t)\mathbbm{1}{\lbrace s_{t} \in \calScom_k\rbrace} \right) \mathbbm{1}_{k}(s_t,\wt{\pi}_k(s_t))\nonumber \\
 &= \underbrace{\sum_{t=t_k}^{t_{k+1}-1} w_k(s_{t+1})\mathbbm{1}{\lbrace s_{t+1} \in \calScom_k\rbrace} - w_k(s_t)\mathbbm{1}{\lbrace s_{t} \in \calScom_k\rbrace}}_{=  w_k(s_{t_{k+1}})\mathbbm{1}{\lbrace s_{t_{k+1}} \in \calScom_k\rbrace} -  w_k(s_{t_k})\mathbbm{1}{\lbrace s_{t_k} \in \calScom_k\rbrace} \leq \rmaxbound \diamcom} \nonumber\\
 &\quad{}+ \sum_{t=t_k}^{t_{k+1}-1} \underbrace{\left(w_k(s_t)\mathbbm{1}{\lbrace s_{t} \in \calScom_k\rbrace} -w_k(s_{t+1})\mathbbm{1}{\lbrace s_{t+1} \in \calScom_k\rbrace}\right)}_{\leq \rmaxbound \diamcom} \mathbbm{1}\lbrace N_k^\pm(s_t,\wt{\pi}_k(s_t))\leq\sqrt{\sfrac{t_k}{SA}}\rbrace\nonumber\\
 &\leq \rmaxbound \diamcom + \rmaxbound \diamcom \sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace \label{eqn:wt_delta_bound_decomposition_4}
\end{align}
By gathering \eqref{eqn:wt_delta_bound_decomposition_1}, \eqref{eqn:wt_delta_bound_decomposition_2}, \eqref{eqn:span_bounded_diameter}, \eqref{eqn:wt_delta_bound_decomposition_3}, \eqref{eqn:mds} and \eqref{eqn:wt_delta_bound_decomposition_4} we obtain the following bound for $\wt{\Delta}_k$:
\begin{align}
        \wt{\Delta}_k
        & \leq 2 \rmaxbound \diamcom \sum_{s,a} \sum_{s'\in\calScom} \underbrace{\mathbbm{1}_{k}(s,a)}_{\leq 1}\underbrace{\nu_k(s,a) \beta_{p,k}^{sas'}}_{\geq 0}   
        + \sum_{t=t_{k}}^{t_{k+1}-1}X_t+\rmaxbound \diamcom \nonumber \\
        &\quad{}+ \rmaxbound (\diamcom+1) \sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace
        + \rmaxbound\sum_{s,a}\underbrace{\frac{\nu_k(s,a)}{\sqrt{t_k}}}_{\geq 0}\underbrace{\mathbbm{1}_{k}(s,a)}_{\leq 1} \nonumber \\ 
        &\leq 2 \rmaxbound \diamcom \sum_{s,a}\sum_{s' \in \calScom} \nu_k(s,a)\beta_{p,k}^{sas'}   + \rmaxbound (\diamcom+1) \sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace \nonumber\\ 
        &\quad{} + \sum_{t=t_{k}}^{t_{k+1}-1}X_t+\rmaxbound \diamcom + \rmaxbound \sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}} \label{eqn:regret_bound_decomposition_2}
\end{align}

\subsection{Summing over episodes with $M^* \in \mathcal{M}_k$ and $t_k \geq C(k)$}\label{sec:regret_bound_sum}

Denote by $\mathbbm{1}(k):=\mathbbm{1}\lbrace t_k \geq C(k)\rbrace \cdot \mathbbm{1}{\lbrace M^* \in \mathcal{M}_{k} \rbrace}$ the indicator function taking value $1$ only when $M^* \in \mathcal{M}_{k}$ and $t_k \geq C(k)$. By gathering \eqref{eqn:regret_bound_decomposition_1} and \eqref{eqn:regret_bound_decomposition_2} we obtain:
{
\allowdisplaybreaks
\begin{align}
 \sum_{k=1}^{m}\Delta_k  \cdot \mathbbm{1}(k) \leq 
 ~&\sum_{k=1}^{m}\wt{\Delta}_k \cdot \mathbbm{1}(k) + 2 \sum_{k=1}^{m}\sum_{s,a}{\nu_k(s,a)\beta_{r,k}^{s,a}}\cdot{ \mathbbm{1}(k)} +  \rmaxbound \sum_{k=1}^{m}\sum_{s,a}{\frac{\nu_k(s,a)}{\sqrt{t_k}}}\cdot{ \mathbbm{1}(k)}\nonumber\\
 \leq ~&2 \rmaxbound \diamcom \sum_{k=1}^{m}\underbrace{ \mathbbm{1}(k)}_{\leq 1}\underbrace{\sum_{s,a} \sum_{s' \in \calScom}\nu_k(s,a)\beta_{p,k}^{sas'}}_{\geq 0} + 2 \sum_{k=1}^{m}\sum_{s,a}\underbrace{\nu_k(s,a)\beta_{r,k}^{s,a}}_{\geq 0}\cdot\underbrace{ \mathbbm{1}(k)}_{\leq 1}\nonumber\\
 &+ \rmaxbound (\diamcom+1) \sum_{k=1}^{m}\underbrace{ \mathbbm{1}(k)}_{\leq 1}\underbrace{\sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace}_{\geq 0}\nonumber\\
 &+ \sum_{t=1}^{T}X_t \mathbbm{1}({k_t})+ \sum_{k=1}^{m}\underbrace{ \mathbbm{1}(k)}_{\leq 1} \underbrace{\rmaxbound \diamcom}_{\geq 0} + 2\rmaxbound \sum_{k=1}^{m}\underbrace{ \mathbbm{1}(t)}_{\leq 1}\underbrace{\sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}}}_{\geq 0}\nonumber\\
 \begin{split}\label{eqn:remaining_terms_regret}
         \leq ~& 2 \rmaxbound \diamcom \sum_{k=1}^{m} \sum_{s,a} \sum_{s' \in \calScom}\nu_k(s,a)\beta_{p,k}^{sas'} + 2 \sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\beta_{r,k}^{s,a}\\
 &+ \rmaxbound (\diamcom+1) \sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace\\
 &+ \sum_{t=1}^{T}X_t \mathbbm{1}({k_t}) + 2\rmaxbound \sum_{k=1}^{m}\sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}} + m\rmaxbound \diamcom
 \end{split}
\end{align}
}
In the remainder of this section, we upper-bound the six terms appearing in \eqref{eqn:remaining_terms_regret}. The main novelty of \eqref{eqn:remaining_terms_regret} compared to \ucrl is the term $ \sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace$ which is not present in the proof of \citet{Jaksch10}. We will show in the next subsection that this term is bounded by $O(\sqrt{SAT})$. All the other terms are similar to those found in \ucrl.

\subsubsection{Poorly visited state-action pairs}
\label{sec:poorly.visited.states}

We first notice that by definition $t_{k_t}\leq t$ where $k_t := \sup \lbrace k \geq 1:~~ t_k \leq t\rbrace$ is the current episode at time $t$.
As a result,
\begin{align*}
  \mathbbm{1}\left\{  N_{k_t}^{\pm}(s_t,a_t) \leq \sqrt{\sfrac{t_{k_t}}{SA}}\right\} \leq \mathbbm{1}\left\{  N_{k_t}^{\pm}(s_t,a_t) \leq \sqrt{\sfrac{t}{SA}} \right\}
\end{align*}
Instead of directly bounding $\sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^{\pm}(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace$ we will bound the number of visits $Z_T$ in state-action pairs that have been visited less than $\sqrt{\sfrac{t}{SA}}$ times
\begin{align*}
        Z_T 
        := \sum_{t=1}^{T}\mathbbm{1}\left\{ N_{k_t}^\pm(s_t,a_t) \leq \sqrt{\sfrac{t}{SA}} \right\}
        \geq &\sum_{t=1}^{T}\mathbbm{1}\left\{  N_{k_t}^\pm(s_t,a_t)\leq \sqrt{\sfrac{t_{k_t}}{SA}} \right\} \\
        &= \sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\mathbbm{1} \left\{  N_k^\pm(s,a) \leq\sqrt{\sfrac{t_k}{SA}} \right\}
\end{align*}
Note that the quantity $N_{k}(s,a)$ is updated only after the end of episode $k$.
Moreover, for all $(s,a) \notin \calScom \times \mathcal{A}$, $\nu_k(s,a) = 0$ implying that only the states $s\in \Scom$ should be considered in the above sums.
Using \eqref{eqn:stopping_condition_ineuality}, we prove the following lemma:
\begin{lemma}\label{lem:bound_bad_state_action}
 For any $T \geq 1$ and any sequence of states and actions $\lbrace s_1, a_1, \dots \dots s_T, a_T \rbrace$ we have:
 \begin{align*}
    Z_T \leq 2\sqrt{\Scom AT} +2\Scom A.
 \end{align*}
\end{lemma}
\begin{proof}
For any episode $k$ starting at time $t_k$, and for any state-action pair $(s,a)$ we recall that $N_k(s,a)$ denotes the number of visits in $(s,a)$ prior to episode $k$ ($k$ not included) and by $\nu_k(s,a)$ the number of visits in $(s,a)$ during episode $k$: % (see \eqref{eqn:N_nu}).
\begin{align*}
 N_{k}(s,a) := \sum_{t=1}^{t_k-1}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace ~~ &\text{and} ~~
 \nu_k(s,a) := \sum_{t=t_k}^{t_{k+1}-1}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace\\
 \implies N_{k}(s,a) &= \sum_{i=1}^{k-1}\nu_i(s,a)
\end{align*}
By convention, we denote by $N_{k_T+1}(s,a):= \sum_{t=1}^{T}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace$ the total number of visits in $(s,a)$ after $T$ time steps ($T$ included).
 We first decompose $Z_T$ as:
 \begin{align*}
         &Z_T := \sum_{s,a} \sum_{t=1}^{T} \mathbbm{1}\Big\{ \max \lbrace 1, N_{k_t}(s,a)-1 \rbrace\leq \sqrt{\sfrac{t}{SA}}\Big\} \cdot \mathbbm{1}\Big\{ (s_t,a_t)= (s,a) \Big\} = \sum_{s \in \Scom} \sum_a Z_T(s,a)\\\
         &\text{where}~~ Z_T(s,a) :=  \sum_{t=1}^{T} \mathbbm{1}\Big\{ \max \lbrace 1, N_{k_t}(s,a)-1 \rbrace\leq \sqrt{\sfrac{t}{SA}}\Big\} \cdot \mathbbm{1}\Big\{ (s_t,a_t)= (s,a) \Big\}
 \end{align*}
 Using the fact that for all $t\geq 1$, $t_{k_t} \leq t \leq t_{k_t +1} -1$ we have:
 \begin{align}
         \forall T\geq \tau\geq 1, ~~ Z_{\tau}(s,a)
         &=\sum_{t=1}^{\tau} \underbrace{\mathbbm{1}\Big\{ \max \lbrace 1, N_{k_t}(s,a)-1 \rbrace\leq \sqrt{\sfrac{t}{SA}}\Big\}}_{\leq 1} \cdot \underbrace{\mathbbm{1}\lbrace (s_t,a_t)= (s,a)\rbrace}_{\geq 0} \nonumber \\
         &\leq \sum_{t=1}^{\tau} \mathbbm{1}\lbrace (s_t,a_t)=(s,a)\rbrace\nonumber \leq  \sum_{t=1}^{t_{k_\tau +1} -1} \mathbbm{1}\lbrace (s_t,a_t)= (s,a)\rbrace \\
         &= N_{k_{\tau} + 1}(s,a) \label{eqn:D_less_N}
%          &\leq \max \lbrace 1,N_{k_{\tau} + 1}(s,a) -1\rbrace +1 \label{eqn:D_less_N}
 \end{align}
 Let's define $t_{s,a}$ as the last time that $Z_t(s,a)$ was incremented by $1$:
 \begin{align*}
         t_{s,a}&:= \max \Big\{ T\geq t\geq 1: \max \lbrace 1, N_{k_t}(s,a)-1 \rbrace\leq \sqrt{\sfrac{t}{SA}} ~~ \text{and} ~~ (s_t,a_t)= (s,a) \Big\} \\
                &~=\min \Big\{ T\geq t\geq 1: Z_{t}(s,a) = Z_T(s,a) \Big\} 
 \end{align*}
 We denote by $m_{s,a}:= k_{t_{s,a}}$ the corresponding episode. By definition,
 \begin{align}\label{eqn:expand_D_T_s_a}
  Z_T(s,a)=Z_{t_{s,a}}(s,a)
 \end{align}
 and
  \begin{align}\label{eqn:bound2_N_m_s_a}
  \max \lbrace 1, N_{m_{s,a}}(s,a)-1 \rbrace\leq \sqrt{\sfrac{t_{s,a}}{SA}}
 \end{align}
 Using \eqref{eqn:D_less_N} with $\tau = t_{s,a}$ we obtain:
 \begin{align}\label{eqn:bound_D_t_s_a}
  Z_{t_{s,a}} \leq N_{m_{s,a}+1}(s,a)
 \end{align}
 Moreover, by definition of $N_k(s,a)$ and \eqref{eqn:stopping_condition_ineuality}:
 \begin{align}
  &N_{m_{s,a}+1}(s,a) = N_{m_{s,a}}(s,a) + \underbrace{\nu_{m_{s,a}}(s,a)}_{\leq  N_{m_{s,a}}^+(s,a) } \leq 2  \underbrace{\max \lbrace 1, N_{m_{s,a}}(s,a) \rbrace}_{\mathclap \leq ~\max \lbrace 1, N_{m_{s,a}}(s,a) -1 \rbrace +1}   \nonumber\\
  &\implies  N_{m_{s,a}+1}(s,a) \leq 2\cdot  \max \lbrace 1, N_{m_{s,a}}(s,a) - 1 \rbrace + 2\label{eqn:bound1_N_m_s_a} 
 \end{align}
%  Since at $t = t_{s,a}$, $D_t(s,a)$ was incremented by $1$ (by definition of $t_{s,a}$) it means that necessarily $\mathbbm{1}\lbrace N_{m_{s,a}}(s,a)\leq \sqrt{t_{s,a}/SA}\rbrace = 1$ (by definition of $D_t(s,a)$) or in other words:
 Gathering \eqref{eqn:expand_D_T_s_a}, \eqref{eqn:bound2_N_m_s_a}, \eqref{eqn:bound_D_t_s_a}, and \eqref{eqn:bound1_N_m_s_a} we obtain:
 \begin{align*}
    Z_T(s,a) = {Z_{t_{s,a}}(s,a)} &\leq {\max \lbrace 1, N_{m_{s,a}+1}(s,a)-1\rbrace} + 1 \leq 2 \cdot {\max \lbrace 1, N_{m_{s,a}}(s,a) - 1\rbrace} +2\\
    &\leq 2 \sqrt{\sfrac{t_{s,a}}{SA}}+2 \\ &\leq  2 \sqrt{\sfrac{T}{SA}} +2 \\
    \implies Z_T &= \sum_{s \in \Scom} \sum_{a} Z_T(s,a) \leq 2 \sqrt{\Scom AT} + 2\Scom A
 \end{align*}
 where for the last inequality we used the fact that $\Scom \leq S$ (by definition) implying \[\Scom/\sqrt{S} = \sqrt{\Scom/S} \cdot \sqrt{\Scom} \leq \sqrt{\Scom}\]
 This concludes the proof.
\end{proof}
As a consequence of Lem.~\ref{lem:bound_bad_state_action}:
\begin{align}\label{eqn:bound_bad_states}
        \sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^\pm(s,a)\leq\sqrt{\sfrac{t_k}{\Scom A}}\rbrace \leq Z_T \leq 2 \sqrt{\Scom AT} + 2\Scom A
\end{align}

\subsubsection{Confidence bounds $\beta_{r,k}^{sa}$ and $\beta_{p,k}^{sas'}$} The first two terms in \eqref{eqn:remaining_terms_regret} involve the confidence bounds on the rewards $\beta_{r,k}^{sa}$ and transition probabilities $\beta_{p,k}^{sas'}$ of the true MDP. These terms can be expanded as follows:
\begin{align*}
 \sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\beta_{r,k}^{sa} 
 &= \sum_{k=1}^{m}\sum_{s,a}\Bigg[\underbrace{\sqrt{14 \wh{\sigma}_{r,k}^2 \ln\left(\frac{2SAt_k}{\delta} \right)}}_{\leq \rmaxbound\sqrt{14 \ln\left(\frac{2SAT}{\delta} \right)}}\frac{\nu_k(s,a)}{\sqrt{N_k^+(s,a)}} \\ 
 &\qquad\qquad\qquad{}+ \frac{49}{3}\rmaxbound \underbrace{\ln\left(\frac{2SAt_k}{\delta} \right)}_{\leq \ln\left(\frac{2SAT}{\delta} \right)} \frac{\nu_k(s,a)}{N_k^\pm(s,a)} \Bigg]\\
 &\leq \rmaxbound\sqrt{14 \ln\left(\frac{2SAT}{\delta} \right)} \sum_{k=1}^{m}\sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{ N_k^+(s,a) }} \\
 &\qquad\qquad\qquad{}+ \frac{49}{3}\rmaxbound \ln\left(\frac{2SAT}{\delta} \right) \sum_{k=1}^{m}\sum_{s,a}\frac{\nu_k(s,a)}{ N_k^\pm(s,a)}
\end{align*}
and similarly
\begin{align*}
        \sum_{k=1}^{m}\sum_{s,a, s'\in\calScom}\nu_k(s,a)\beta_{p,k}^{sas'} \leq 
        &\sqrt{14 \ln\left(\frac{2SAT}{\delta} \right)} \sum_{k=1}^{m}\sum_{s,a} \sum_{s'\in\calScom}\nu_k(s,a)\sqrt{\frac{\wh{p}_k(s'|s,a)(1-\wh{p}_k(s'|s,a))}{ N_k^+(s,a)}}  \\ 
        &+ \frac{49}{3} \Scom \ln\left(\frac{2SAT}{\delta} \right) \sum_{k=1}^{m}\sum_{s,a}\frac{\nu_k(s,a)}{ N_k^\pm(s,a)}
\end{align*}
The sum $\sum_{s' \in \calScom} \sqrt{\wh{p}_k(s'|s,a)(1-\wh{p}_k(s'|s,a))}$ can be bounded by $\sqrt{\nextstatescom-1}$ as in~\citep[Appendix F.7]{fruit2018constrained} where $\nextstatescom$ is the maximal support over all state-action pairs $(s,a)$
\begin{align*}
        \nextstatescom = \max_{(s,a) \in \calScom \times \mathcal{A}} \|p(\cdot|s,a)\|_0 %\big|\supp \lbrace {p}(\cdot|s,a) \rbrace\big|
\end{align*}
% with $\supp \lbrace p(\cdot|s,a) \rbrace =  \lbrace s' \in \mathcal{S}: ~ p(s'|s,a)>0 \rbrace$ the support of $p(\cdot|s,a)$ and $|\cdot|$ denotes the cardinal of a set.\\ 
with $\|\cdot\|_0$ is the $\ell_0$-norm counting the non-zero elements in the vector $p(\cdot|s,a)$.
Note that we have restricted the maximization over $(s,a) \in \calScom \times \A$ since $\nu_k(s,a) = 0$ for any other pair.
Since \eqref{eqn:stopping_condition_ineuality} holds, Lemma 19 of \citet{Jaksch10} can still be applied. 
Moreover, exploiting again the fact that for all $(s,a) \notin \calScom \times \mathcal{A}$, $\nu_k(s,a) = 0$ and as a result we obtain 
\begin{align}\label{eqn:nu_over_sqrt_N}
 \sum_{k=1}^{m}\sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}} \leq \sum_{k=1}^{m}\sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{N_k^+(s,a)}} \leq \left(\sqrt{2} +1 \right)\sqrt{\Scom AT}
\end{align}
and as shown in~\citep[Appendix F.7]{fruit2018constrained} (with the difference that $S$ is restricted to $\Scom$) we have:
\begin{align}\label{eqn:nu_over_N}
 \sum_{k=1}^{m}\sum_{s,a} \frac{\nu_k(s,a)}{N_k^\pm(s,a)} \leq 6\Scom A + 2\Scom A\ln(T)
\end{align}

\subsubsection{Martingale Difference Sequence $X_t\cdot\mathbbm{1}({k_{t}})$}
In Sec.~\ref{sec:bound_wt_delta} we already proved that $(X_t,\mathcal{F}_t)_{t\geq 1}$ is an MDS \ie for all $t\geq 1$, $\mathbbm{E}[X_{t}|\mathcal{F}_{t-1}]=0$. Since $k_t$ is $\mathcal{F}_{t-1}$-measurable, we have \[\mathbbm{E}[X_{t}\mathbbm{1}({k_{t}})|\mathcal{F}_{t-1}]= \mathbbm{1}({k_{t}})\cdot\mathbbm{E}[X_{t}|\mathcal{F}_{t-1}] = 0\]
Therefore, $(X_t\mathbbm{1}({k_{t}}),\mathcal{F}_t)_{t\geq 1}$ is also an MDS. By Azuma's inequality (see for example \citep[Lemma 10]{Jaksch10}):
\begin{align}
\mathbb{P}\left(\sum_{t=1}^{T} X_t\mathbbm{1}({k_{t}}) >  \rmaxbound \diamcom \sqrt{\frac{5}{2} T \ln\left(\frac{8T}{\delta}\right)} \right) \leq \left(\frac{\delta}{8T}\right)^{5/4} < \frac{\delta}{12T^{5/4}} \nonumber\\
\implies \sum_{t=1}^{T} X_t\mathbbm{1}({k_{t}}) \leq  \rmaxbound \diamcom \sqrt{\frac{5}{2} T \ln\left(\frac{8T}{\delta}\right)} ~~ \text{w.p.}\geq 1-\frac{\delta}{12T^{5/4}} \label{eqn:bound_martingale}
\end{align}

\subsubsection{Number of episodes}\label{app:regret.number.episodes}
The stopping condition of episodes used by \tucrl (see Alg.~\ref{fig:ucrl.constrained}) combines the original stopping condition of \ucrl with the condition $s_t \in \calStrans_{k_t}$. Using only inequality \eqref{eqn:stopping_condition_ineuality}, \citet[Figure 1]{Jaksch10} proved that for any any sequence $\lbrace s_1,a_1, \dots, s_{T},a_T\rbrace$, the number of episodes is bounded by $1 +2SA + SA \log_2\left( \frac{T}{SA} \right)$.
Since \eqref{eqn:stopping_condition_ineuality} also holds in our case, the total number of episodes $m$ after $T$ time steps can be bounded by the same quantity (with $S$ replaced by $\Scom$ since sates in $\calStrans$ will never be visited) plus the number of times the event $s_t \in  \calStrans_{k_t}$ occurs. Since whenever $s_t \in \calStrans_{k_t}$ state $s_t$ is removed from $\calStrans_{k_t+1}$ and $s_t$ necessarily belongs to $\calScom$ (by definition), this event can happen at most $\calScom$ times. By Proposition 18 in~\citep{Jaksch10} we thus have:
\begin{align}\label{eqn:nb_episodes}
 m \leq 1 +2\Scom A + \Scom A \log_2\left( \frac{T}{\Scom A} \right) + \Scom
\end{align}

\subsubsection{Conclusion}
By gathering \eqref{eqn:remaining_terms_regret}, \eqref{eqn:bound_bad_states}, \eqref{eqn:nu_over_sqrt_N}, \eqref{eqn:nu_over_N}, \eqref{eqn:bound_martingale} and \eqref{eqn:nb_episodes} we conclude that with probability at least $1-\frac{\delta}{12T^{5/4}}$:
\begin{align}
 \begin{split}\label{eqn:final_bound_delta}
 \sum_{k=1}^{m}\Delta_k  \cdot \mathbbm{1}(k) \leq ~& 2 \left(\sqrt{28} +\sqrt{14} \right) \rmaxbound \diamcom \sqrt{ (\nextstatescom-1)\Scom AT \ln\left(\frac{2SAT}{\delta} \right)} \\
                                                    &+ \frac{196}{3}\rmaxbound \diamcom \left(\Scom\right)^2 A \ln\left(\frac{2SAT}{\delta} \right)(3+ \ln(T)) \\&+ 2\left(\sqrt{28} +\sqrt{14} \right) \rmaxbound\sqrt{\Scom AT\ln\left(\frac{2SAT}{\delta} \right)} \\ 
 &+ \frac{196}{3}\rmaxbound \Scom A \ln\left(\frac{2SAT}{\delta} \right) (3 + \ln(T))\\& + 2 \rmaxbound (\diamcom+1) (\sqrt{\Scom AT}+\Scom A)\\
 &+ \rmaxbound \diamcom \sqrt{\frac{5}{2} T \ln\left(\frac{8T}{\delta}\right)}  + 2\left(\sqrt{2} +1 \right)\rmaxbound\sqrt{\Scom AT} \\&+ \rmaxbound \diamcom \left(1 +2\Scom A + \Scom A \log_2\left( \frac{T}{SA} \right) + \Scom  \right)\\
 \leq& C\cdot\left(\rmaxbound \diamcom \sqrt{\nextstatescom \Scom AT \ln\left( \frac{SAT}{\delta} \right)} + \rmaxbound \diamcom \left(\Scom\right)^2 A \ln^2\left( \frac{SAT}{\delta} \right) \right)
 \end{split}
\end{align}
where $C$ is a numerical constant independent of the MDP instance.

\subsection{Completing the regret bound}

From \eqref{eqn:martingale_reward}, with probability at least $1-\frac{\delta}{12T^{5/4}}$:
\begin{align*}
 \Delta(\tucrl,T) &\leq \sum_{k=1}^{m}\Delta_k + \rmaxbound \sqrt{\frac{5}{2} T \ln\left(\frac{8T}{\delta}\right)}\\& = \underbrace{\sum_{k=1}^{m}\Delta_k\mathbbm{1}(k)}_{\text{see~\eqref{eqn:final_bound_delta}}} + \sum_{k=1}^{m}\Delta_k\cdot(1-\mathbbm{1}(k)) + \rmaxbound \sqrt{\frac{5}{2} T \ln\left(\frac{8T}{\delta}\right)}
\end{align*}
where $1-\mathbbm{1}(k)$ is the complement of $\mathbbm{1}(k)$ \ie takes value $1$ only when $t_k < C(k)$ (see \eqref{eqn:def_f}) \underline{{or}} $M^* \notin \mathcal{M}_{k}$. By Boole's inequality: \[1-\mathbbm{1}(k) \leq \mathbbm{1}\lbrace M^* \notin \mathcal{M}_{k} \rbrace +  \mathbbm{1}\lbrace t_k < C(k) \rbrace\]
and so
\begin{align*}
 \sum_{k=1}^{m}\Delta_k\cdot(1-\mathbbm{1}(k)) \leq  \underbrace{\sum_{k=1}^{m}\Delta_k\cdot\mathbbm{1}\lbrace M^* \notin \mathcal{M}_{k} \rbrace}_{\text{see~\eqref{eqn:failed_episodes}}} + \underbrace{\sum_{k=1}^{m}\Delta_k\cdot\mathbbm{1}\lbrace t_k < C(k) \rbrace }_{\text{see~\eqref{eqn:regret_bound_first_episodes}}}
\end{align*}
% By definition for all $ k \geq 1$, \[\Delta_k = \sum_{t=t_k}^{t_{k+1}-1}\left(g^*-r(s_t,a_t)\right) \leq \rmaxbound(t_{k+1}-t_k)\] and as a consequence of \eqref{eqn:stopping_condition_ineuality} \[t_{k+1} = t_k + \sum_{s,a}\underbrace{\nu_k(s,a)}_{\leq N_k(s,a)} \leq  t_k+\sum_{s,a}N_k(s,a) = 2t_k \]
% Defining $k^* = \max \lbrace k \geq 1 : ~ t_k < D^2 S^3 A \rbrace$ we have
% \begin{align*}
%  \sum_{k=1}^{m}\Delta_k\cdot\underbrace{\mathbbm{1}\lbrace t_k < D^2 S^3 A \ln(...) \rbrace}_{\geq 0} &\leq \rmaxbound \sum_{k=1}^{m}(t_{k+1}-t_k)\cdot\mathbbm{1}\lbrace t_k < D^2 S^3 A \ln(...) \rbrace \\
%  &\leq \rmaxbound \sum_{k=1}^{k^*}(t_{k+1}-t_k) = \rmaxbound ( t_{k^*+1} -1) \leq 2\rmaxbound t_{k^*}\\
%  &\leq  2 \rmaxbound D^2 S^3 A \ln(...) ~~ \text{by definition of }~k^*
% \end{align*}
In conclusion, there exists a numerical constant $C$ independent of the MDP instance such that for any MDP and any $T>1$, with probability at least $1 - \frac{\delta}{12T^{5/4}} - \frac{\delta}{12T^{5/4}}- \frac{\delta}{12T^{5/4}} = 1 - \frac{\delta}{4T^{5/4}}$ we have:
\begin{align}\label{eqn:final_bound_regret}
        \Delta(\tucrl,T) &\leq C\cdot\left(\rmaxbound \diamcom \sqrt{\nextstates \Scom A T \ln\left( \frac{SAT}{\delta} \right)} + \rmaxbound \left(\diamcom\right)^2 S^3 A \ln^2\left( \frac{SAT}{\delta} \right) \right)
\end{align}
Since $\sum_{T=2}^{+\infty}\frac{\delta}{4T^{5/4}}=  \delta$, by taking a union bound we have that the regret bound \eqref{eqn:final_bound_regret} holds with probability at least $1-\delta$ for all $T>1$.



==> app_tucrl_desc.tex <==
% !TEX root = tucrl.tex

\section{Description of \tucrl}\label{app:tucrl.description}
In this section we provide a detailed description of \tucrl and it is meant to be a complement to Sec.~\ref{sec:tucrl} in the main paper.

Similarly to \ucrl, \tucrl proceeds through episodes $k=1,2,\dots$. We index episodes by $k$ as is done in \citep{Jaksch10}.
Episode $k$ starts at time $t_k$, and for any state-action pair $(s,a)$ we denote by $N_k(s,a)$ the number of visits in $(s,a)$ prior to episode $k$ ($k$ not included) and by $\nu_k(s,a)$ the number of visits in $(s,a)$ during episode $k$:
\begin{align}\label{eqn:N_nu}
\begin{split}
 N_{k}(s,a) := \sum_{t=1}^{t_k-1}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace~~ &\text{and} ~~
 \nu_k(s,a) := \sum_{t=t_k}^{t_{k+1}-1}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace\\
 \implies N_{k}&(s,a) = \sum_{i=1}^{k-1}\nu_i(s,a)
 \end{split}
\end{align}
By convention, we denote by $N_{k_T+1}(s,a):= \sum_{t=1}^{T}\mathbbm{1}\lbrace (s_t,a_t)= (s,a) \rbrace$ the total number of visits in $(s,a)$ up to time $T$ ($T$ included). We will also use the convenient notations $N_k^+(s,a):= \max\lbrace 1,N_k(s,a)\rbrace$ and $N_k^\pm(s,a):= \max\lbrace 1,N_k(s,a)-1\rbrace$ for the maximum value between $1$ and $N_k(s,a)$ or $N_k(s,a)-1$.
This term will frequently appear in the proof (App.~\ref{app:tucrl.regret}). The stopping condition of episodes used by \tucrl implies that (see Alg.~\ref{fig:ucrl.constrained}):
\begin{align}\label{eqn:stopping_condition_ineuality}
 \forall k \geq 1, ~\forall (s,a) \in \calS \times \A, ~~ \nu_{k}(s,a) \leq N_k^+(s,a)
\end{align}


\paragraph{\ucrl.} We start describing \ucrl since \tucrl leverages on its idea.
At the beginning of each episode $k$, \ucrl computes a set of plausible MDPs defined as
\begin{equation}
        \label{eq:plausible.mdps}
        \begin{aligned}
                \mathcal M_k^1 = \big\{ M = \langle \calS, \A, \wt{r}, \wt{p}\rangle \;:\; &\forall (s,a)\in \calS \times \A,~\wt{r}(s,a) \in B_{r,k}^1(s,a),\\
                                                                                           &\wt{p}(s'|s,a) \in B_{p,k}^1(s,a,s'),~ \wt{p}(\cdot|s,a) \in \mathcal{C}
                \big\}
        \end{aligned}
\end{equation}
where $\mathcal{C} = \{p \in \mathbb{R}^S | \forall s,~p(s) \geq 0 \wedge \sum_{s} p(s) = 1\}$ is the $(S-1)$-simplex, $B_{r,k}^1$ and $B_{p,k}^1$ are high-probability confidence intervals on the rewards and transition probabilities of the true MDP $M^*$, which guarantees that $M^* \in \mathcal{M}_k^1$ w.h.p.
In this paper we use confidence intervals constructed using the empirical Bernstein's inequality~\citep{audibert2007tuning,Maurer2009empirical}
\begin{align*}
\beta_{r,k}^{sa}
:=
         \sqrt{\frac{14 
                         \wh{\sigma}_{r,k}^2(s,a)
%        \ln(2 SA t_k/\delta)
                        b_{k,\delta}
                }{
%        \max\lbrace 1, N_k(s,a)\rbrace
        N^{+}_k(s,a)
}} + \frac{\frac{49}{3}
%                 \alpha_r 
\rmaxbound
%        \ln(2 SA t_k/\delta)
        b_{k,\delta}
        }{
        N^{\pm}_k(s,a)
%        \max\lbrace 1, N_k(s,a)-1 \rbrace
}
, \qquad
\beta_{p,k}^{sas'}
:= 
\sqrt{\frac{14 \wh{\sigma}_{p,k}^2(s'|s,a) 
%        \ln(2 SA t_k/\delta)
                        b_{k,\delta}
                }{
%        \max\lbrace 1, N_k(s,a)\rbrace
        N^{+}_k(s,a)
}
} +\frac{\frac{49}{3}
%                 \alpha_p 
%        \ln(2 SA t_k/\delta)
        b_{k,\delta}
        }{
        N^{\pm}_k(s,a)
%        \max\lbrace 1,N_k(s,a)-1 \rbrace
}
\end{align*}
where $N_k(s,a)$ is the number of visits in $(s, a)$ before episode $k$, 
$N^{+}_k(s,a) := \max\lbrace 1, N_k(s,a) \rbrace$, 
$N^{\pm}_k(s,a) := \max\lbrace 1, N_k(s,a)-1 \rbrace$, 
$\wh{\sigma}_{r,k}^2(s,a)$ and $\wh{\sigma}_{p,k}^2(s'|s,a)$ are the empirical variances of $r(s,a)$ and ${p}(s'|s,a)$ %respectively 
% (formally defined in eqn.~\eqref{eqn:def_empirical_variance} of App.~\ref{app:regret.reg.ucrl}) 
and $b_{k,\delta} = \ln(2 SA t_k/\delta)$.
%
Given the empirical averages $\wh{r}_k(s,a)$ and $\wh{p}_k(s'|s,a)$ of rewards and transitions, we define $\mathcal{M}_k^1$ by $B_{r,k}^1(s,a) := [\wh{r}_k(s,a) - \beta_{r,k}^{sa}, \wh{r}_k(s,a) + \beta_{r,k}^{sa}] \cap [0, \rmaxbound]$ and $B_{p,k}^1(s,a,s') := [\wh{p}_k(s'|s,a) - \beta_{p,k}^{sas'},\wh{p}_k(s'|s,a) + \beta_{p,k}^{sas'}] \cap [0,1]$.

Once $\mathcal{M}_k^1$ has been computed, \ucrl finds an approximate solution $(\wt{M}_k^*,\wt\pi_k^*)$ to the problem:
%
\begin{align}\label{eq:ucrl.optimization_app}
( \wt{M}^*_k, \wt\pi^*_k ) \in \argmax_{M\in\mathcal{M}_k, \pi\in\SD(M)} g^\pi_M.
\end{align}


\paragraph{\tucrl.} At each episode $k$, \tucrl computes the empirical estimates of $\calScom$ and $\calStrans$ \ie the set of communicating and transient states in $M^*$:
\begin{align*}
        \calScom_k := \left\{s \in \calS \;\big|\; \sum_{a \in \A_s} N_k(s,a) > 0 \right\} \cup \{s_{t_k}\}, \qquad\quad
        \calStrans_k := \calS \setminus \calScom_k.
\end{align*}
%
Then, \tucrl builds a set of \emph{constrained} MDPs $\mathcal{M}_k^2$ (see Eq.~\ref{eq:plausible.mdps}) such that $B_{r,k}^2(s,a) = B_{r,k}^1(s,a),\; \forall (s,a) \in \calS \times \A$ and, $\forall (s,a,s') \in \calS \times \A \times \calS$:
\begin{equation*}
        B_{p,k}^2(s,a,s') = \begin{cases}
                \{0\} & \text{if } (s,a,s') \in \left( (\calS \times \A) \setminus \mathcal{K} \right) \times \calStrans_k\\
                B_{p,k}^1(s,a,s') & \text{otherwise} % \forall (s,a,s') \in \{\calS \times \A \times \calScom_k\} \cup \{(\mathcal{K} \cup (\calStrans_k \times \A)) \times \calStrans_k \}
        \end{cases}
\end{equation*}
where $\mathcal{K} = \Big\{ (s,a) \in \calScom_k \times \A \,:\, N_k^\pm(s,a) \leq \sqrt{\sfrac{t_k}{SA}} \Big\}$ contains the state-action pairs that are currently non-sufficiently explored.
For these pairs, it is \emph{plausible} it may exist a transition to a state $s'$ that has never been observed (\ie $s' \in \calStrans_k$).

Finally, we introduce \emph{relaxations} of the extended MDPs that consider the $\ell_1$-norm concentration inequality around $p(\cdot|s,a)$ instead of $S$ concentration inequalities around $p(s'|s,a)$ for all $s'\in \calS$.
We will denote by $\mathcal{M}^{1+}_k$ and  $\mathcal{M}_k^{2+}$ the relaxation of $\mathcal{M}_k^1$ and $\mathcal{M}_k^2$, respectively.
Then, for $i \in \{1,2\}$, 
$\mathcal{M}_k^{i+} = \Big\{ M = (\calS,\A, \wt{r}, \wt{p}) :\;
        \wt{r}(s,a) \in B_{r,k}^{i+}(s,a), \;
                        \wt{p}(\cdot|s,a) \in B_{p,k}^{i+}(s,a) \Big\}$
where the reward intervals are not altered (\ie $B_{r,k}^{i+} = B_{r,k}^{i}$) and, for any $(s,a) \in \calS \times \A$
\begin{align*}
        B_{p,k}^{1+}(s,a) 
        &= \left\{ 
                \wt{p}(\cdot|s,a)\in \mathcal{C} :~
%                \wt{p}\in \mathbb{R}^S :~ \wt{p}(\cdot|s,a)\in \mathcal{C} \wedge
                \| \wt{p}(\cdot|s,a) - \wh{p}(\cdot|s,a) \|_1 \leq \beta_{p,k}^{sa} := \sum_{s'\in\calS}\beta_{p,k}^{sas'}
        \right\},\\
        B_{p,k}^{2+}(s,a) 
        &= \begin{cases}
        B_{p,k}^{1+}(s,a) \cap \left\{\wt{p} \in \mathcal{C} :~ \sum_{s' \in \calStrans_k} \wt{p}(s'|s,a) = 0  \right\} & \text{if }(s,a) \in \mathcal{K}\\
                B_{p,k}^{1+}(s,a) & \text{otherwise} %(s,a) \in (\calS \times \A) \setminus \mathcal{K}\\
        \end{cases}
\end{align*}

Then, \tucrl considers a variation of problem~\eqref{eq:ucrl.optimization_app} defined as:
%At each episode $k$, \tucrl consider a slightly modify problem~\eqref{eq:ucrl.optimization} as follows:
\begin{equation}
        \label{eq:tucrl.optimization_app}
        (\wt{M}_k, \wt{\pi}_k) = \argmax_{M \in \mathcal{M}_k^\diamond, \pi \in \Pi^{\textsc{SD}}(M)} \{g^{\pi}_M\} 
        \qquad \text{where } \quad \mathcal{M}_k^\diamond = \begin{cases}
                \mathcal{M}_k^{2} & \text{if } \calStrans_k = \emptyset\\
                \mathcal{M}_k^{2+} & \text{otherwise}
        \end{cases}
\end{equation}
%
Similarly to \ucrl, problem~\eqref{eq:tucrl.optimization_app} is equivalent to finding $\wt{\mu}^* \in \argmax_{\mu \in \SD(\wt{\mathcal{M}}_k)} \big\lbrace g^\mu_{\wt{\mathcal{M}}_k} \big\rbrace$ where $\wt{\mathcal{M}}_k$ is the \emph{extended} MDP (sometimes called \emph{bounded-parameter} MDP) implicitly defined by $\mathcal{M}_k^{\diamond}$.
This problem can be solved up to an $\epsilon_k$-approximation ($\epsilon_k = \rmaxbound/\sqrt{t_k}$) using extended value iteration (EVI) on $\mathcal{M}_k^{\diamond}$.
Starting from an initial vector $u_0 = 0$, EVI iteratively applies the optimal Bellman operator of $\mathcal{M}_k^{\diamond}$: $u_{n+1} = \wt{L}_{\mathcal{M}_k^{\diamond}} u_n$.
Note that when $\calStrans_k = \emptyset$, $\wt{L}_{\mathcal{M}_k^{\diamond}} = \wt{L}_{\mathcal{M}_K^1}$ (see~\citep[][Eq. 5]{Jaksch10}). Otherwise, $\wt{L}_{\mathcal{M}_k^{\diamond}} = \wt{L}_{\mathcal{M}_K^{2+}}$ where, for any $v \in \mathbb{R}^S$:
\begin{equation}\label{eq:Lop_m2plus}
\begin{aligned}
        \wt{L}_{\mathcal{M}_k^{2+}}v(s) &:= \max_{a \in \A_s} \left\{
                \max_{\wt{r} \in B_{r,k}(s,a)} \wt{r} +  (\wt{p}^{sa})^\transp v
        \right\}
\end{aligned}
\end{equation}
and $\wt{p}^{sa} = \argmax_{\wt{p} \in B_{p,k}^{2+}(s,a)} \{\wt{p}^T v_{n}\}$ can be solved using Alg.~\ref{alg:opt.prob.h}:
\begin{align*}
 \wt{p}^{sa} = \begin{cases}
                \textsc{OTP}(\wh{p}(\cdot|s,a), \sum_{s'\in\calS}\beta_{p,k}^{sas'}, u, \calScom_k)	& \text{if}~(s,a) \in \mathcal{K}\\
                \textsc{OTP}(\wh{p}(\cdot|s,a), \sum_{s'\in\calS}\beta_{p,k}^{sas'}, u, \calS)	& \text{otherwise}.
               \end{cases}
\end{align*}



==> sec_algorithm.tex <==
% !TEX root = tucrl.tex

\section{Truncated UCRL}\label{sec:tucrl}
%\begin{itemize}
%        \item Modified Extended MDP
%        \item Optimization
%        \item Regret
%        \item Comment the regret
%        \item Why it works? \eg we rely on Bernstein bound ...
%        \item Put lemma (sum of indicators)
%\end{itemize}
In this section we introduce \tucrl, an optimistic online RL algorithms that is able to efficiently balance exploration and exploitation in order to learn in weakly communicating MDPs without prior knowledge.

At the beginning of each episode \tucrl constructs the empirical estimates of $\calScom$ and $\calStrans$ \ie the set of communicating and transient states in $M^*$:
\begin{align*}
        \calScom_k := \left\{s \in \calS \;\big|\; \sum_{a \in \A_s} N_k(s,a) > 0 \right\} \cup \{s_{t_k}\}, \qquad\quad
        \calStrans_k := \calS \setminus \calScom_k,
\end{align*}
where $t_k$ is the starting time of episode $k$.
Then, \tucrl builds a set of \emph{constrained} MDPs $\mathcal{M}_k^2$ (see Eq.~\ref{eq:plausible.mdps}) such that $B_{r,k}^2(s,a) = B_{r,k}^1(s,a),\; \forall (s,a) \in \calS \times \A$ and, $\forall (s,a,s') \in \calS \times \A \times \calS$:
\begin{equation*}
        B_{p,k}^2(s,a,s') = \begin{cases}
                \{0\} & \text{if } (s,a,s') \in \left( (\calS \times \A) \setminus \mathcal{K} \right) \times \calStrans_k\\
                B_{p,k}^1(s,a,s') & \text{otherwise} % \forall (s,a,s') \in \{\calS \times \A \times \calScom_k\} \cup \{(\mathcal{K} \cup (\calStrans_k \times \A)) \times \calStrans_k \}
        \end{cases}
\end{equation*}
where $\mathcal{K} = \Big\{ (s,a) \in \calScom_k \times \A \,:\, N_k^\pm(s,a) \leq \sqrt{\sfrac{t_k}{SA}} \Big\}$ contains the state-action pairs that are currently non-sufficiently explored.
For these pairs, it is \emph{plausible} it may exist a transition to a state $s'$ that has never been observed (\ie $s' \in \calStrans_k$).

Finally, we introduce \emph{relaxations} of the extended MDPs that consider the $\ell_1$-norm concentration inequality around $p(\cdot|s,a)$ instead of $S$ concentration inequalities around $p(s'|s,a)$ for all $s'\in \calS$.
We will denote by $\mathcal{M}^{1+}_k$ and  $\mathcal{M}_k^{2+}$ the relaxation of $\mathcal{M}_k^1$ and $\mathcal{M}_k^2$, respectively.
Then, for $i \in \{1,2\}$, 
$\mathcal{M}_k^{i+} = \Big\{ M = (\calS,\A, \wt{r}, \wt{p}) :\;
        \wt{r}(s,a) \in B_{r,k}^{i+}(s,a), \;
                        \wt{p}(\cdot|s,a) \in B_{p,k}^{i+}(s,a) \Big\}$
where the reward intervals are not altered (\ie $B_{r,k}^{i+} = B_{r,k}^{i}$) and, for any $(s,a) \in \calS \times \A$
\begin{align*}
        B_{p,k}^{1+}(s,a) 
        &= \left\{ 
                \wt{p}(\cdot|s,a)\in \mathcal{C} :~
%                \wt{p}\in \mathbb{R}^S :~ \wt{p}(\cdot|s,a)\in \mathcal{C} \wedge
                \| \wt{p}(\cdot|s,a) - \wh{p}(\cdot|s,a) \|_1 \leq \beta_{p,k}^{sa} := \sum_{s'\in\calS}\beta_{p,k}^{sas'}
        \right\},\\
        B_{p,k}^{2+}(s,a) 
        &= \begin{cases}
        B_{p,k}^{1+}(s,a) \cap \left\{\wt{p} \in \mathcal{C} :~ \sum_{s' \in \calStrans_k} \wt{p}(s'|s,a) = 0  \right\} & \text{if }(s,a) \in \mathcal{K}\\
                B_{p,k}^{1+}(s,a) & \text{otherwise} %(s,a) \in (\calS \times \A) \setminus \mathcal{K}\\
        \end{cases}
\end{align*}

Then, \tucrl considers a variation of problem~\eqref{eq:ucrl.optimization} defined as:
%At each episode $k$, \tucrl consider a slightly modify problem~\eqref{eq:ucrl.optimization} as follows:
\begin{equation}
        \label{eq:tucrl.optimization}
        (\wt{M}_k, \wt{\pi}_k) = \argmax_{M \in \mathcal{M}_k^\diamond, \pi \in \Pi^{\textsc{SD}}(M)} \{g^{\pi}_M\} 
        \qquad \text{where } \quad \mathcal{M}_k^\diamond = \begin{cases}
                \mathcal{M}_k^{2} & \text{if } \calStrans_k = \emptyset\\
                \mathcal{M}_k^{2+} & \text{otherwise}
        \end{cases}
\end{equation}
%
Similarly to \ucrl, this problem can be solved up to an $\epsilon_k$-approximation ($\epsilon_k = \rmaxbound/\sqrt{t_k}$) using EVI on $\mathcal{M}_k^{\diamond}$ (see Eq.~\ref{eq:evi}).
% Given a vector $u_0 \in \mathbb{R}^S$, EVI iteratively applies the optimal Bellman operator of $\mathcal{M}_k^{\diamond}$. % until the condition  is met. %\footnote{ $sp_{\calScom_k}\left\{u_{n+1} - u_n\right\} := \max_{s\in\calScom_k} \{u_{n+1}(s) - u_{n}(s)\} - \min_{s\in\calScom_k}\{u_{n+1}(s)-u_{n}(s)\}$.}
Note that when $\calStrans_k = \emptyset$, $\wt{L}_{\mathcal{M}_k^{\diamond}} = \wt{L}_{\mathcal{M}_K^1}$. Otherwise, $\wt{L}_{\mathcal{M}_k^{\diamond}} = \wt{L}_{\mathcal{M}_K^{2+}}$ where, for any $v \in \mathbb{R}^S$:
\begin{equation}\label{eq:Lop_m2plus}
\begin{aligned}
        \wt{L}_{\mathcal{M}_k^{2+}}v(s) &:= \max_{a \in \A_s} \left\{
                \max_{\wt{r} \in B_{r,k}(s,a)} \wt{r} +  (\wt{p}^{sa})^\transp v_n
        \right\}
\end{aligned}
\end{equation}
and $\wt{p}^{sa} = \argmax_{\wt{p} \in B_{p,k}^{2+}(s,a)} \{\wt{p}^T v_{n}\}$ can be solved using Fig. 2~\citep{Jaksch10} except when $(s,a) \in \mathcal{K}$ in which case we restrict the algorithm to work on $\calScom_k$ since $\wt{p}^{sa}(s') := 0$ for any $s' \in \calStrans_k$ (see App.~\ref{} and Alg.~\ref{alg:opt.prob.h} for details).
If EVI is stopped when $sp_{\calScom_k}\left\{u_{n+1} - u_n\right\} \leq \epsilon_k$ and the true MDP is sufficiently explored, then the greedy policy $\wt{\mu}_k$ \wrt $u_n$ is $\epsilon_k$-optimal, \ie $g^{\wt{\mu}_k}_{\wt{\mathcal{M}}_k} \geq g^*_{\wt{\mathcal{M}}_k} \geq g^*_{M^*} - \epsilon_k$ (see Sec.~\ref{sec:sketch.regret.proof} for details).
Finally, note that when the true MDP $M^*$ is communicating, there exists an episode $\wb{k}$ \st for all $k \geq \wb{k},~\calStrans_k = \emptyset$ and
\tucrl will behave like \ucrl with the tightest possible confidence intervals (\ie $ \mathcal{M}_k^\diamond =  \mathcal{M}_k^2 =  \mathcal{M}_k^1$).

We are now ready to prove the following regret bound (see App.~\ref{app:tucrl.regret}).

\begin{theorem}\label{thm:tucrl.regret}
        For any weakly communicating MDP $M$, with probability at least $1-\delta$ it holds that for any $T > 1$, the regret of \tucrl is bounded as
        \[
                \Delta(\tucrl,T) = \mathcal{O} \left(\rmaxbound D_c \sqrt{\nextstates SA T \ln\left( \frac{SAT}{\delta} \right)} + \rmaxbound D_c^2 S^3 A \ln^2\left( \frac{SAT}{\delta} \right) \right).
        \]
%        where $C$ is a numerical constant independent of the MDP $M$.
\end{theorem}
\todom{Comments on the regret}

\subsection{Analysis of \tucrl} \label{sec:sketch.regret.proof}
This section aims to provide a rough outline of the main steps required to prove Thm.~\ref{thm:tucrl.regret}.
The analysis of \tucrl is detailed in App.~\ref{app:tucrl.regret} and leverages on the structure used for \ucrl~\citep{Jaksch10}.
The main difference is due to the use of the \emph{truncated} extended MDP $\mathcal{M}_k^{2+}$ which implies that the statistical argument may fail (\ie if $\calStrans_k \neq \emptyset$, the true MDP $M^*$ might not be included in $\mathcal{M}_k^{2+}$). We will show how to treat this case based on the exploration level of an episode $k$.

In particular, 
%\textbf{Linear phase:} 
\tucrl suffers \textbf{linear regret} in all the episodes with a non-sufficient level of exploration (\ie episodes $k$ s.t. $t_k < C(k) = \mathcal{O}\left(D_c^2 S^3A\ln^2(\sfrac{2SAt_k}{\delta})\right)$).
Since the overall number of times this event happens is ``small'', the contribute to the cumulative regret is polylogarithmic: $\sum_{k=1}^m \Delta_k \cdot \mathbbm{1}\lbrace t_k < C(k) \rbrace = \mathcal{O}(\rmaxbound D_c^2S^3A\ln^2\left(\sfrac{2SAT}{\delta}\right))$ where $\Delta_k$ is the regret in episode $k$.
%
Note that 
% \textbf{Number of episodes:}
% Similarly to \ucrl, the cumulative regret $\Delta(\tucrl,T)$ can be bounded w.h.p.\@\xspace by $\sum_{k=1}^m \Delta_k + \rmaxbound\sqrt{\frac{5}{2}T \ln\left(\frac{8T}{\delta}\right)}$ where $\Delta_k = \sum_{s,a} \nu_k(s,a)\left(g^* - r(s,a)\right)$ is the regret in episode $k$ and $\nu_k(s,a)$ is the number of visits in $(s,a)$ during episode $k$.
the stopping condition used by \tucrl is the original \ucrl one combined with the condition $s_{t} \in \calS_{k_t}^2$ ($k_t$ being the episode associated to time $t$). Then, it is easy to prove (see App.~\ref{app:regret.number.episodes}) that the \textbf{total number of episodes} $m$ is incremented at most by $S$.

% \textbf{Optimism:} 
% we start noticing that when $\calStrans_k = \emptyset$, the true MDP $M^* \in \mathcal{M}_k^1 = \mathcal{M}_k^2 = \mathcal{M}_k^\diamond$ w.h.p. and we can use the same arguments in~\citep{Jaksch10}. When $\calStrans_k \neq \emptyset$, $M^*$ might not be included in $\mathcal{M}_k^\diamond = \mathcal{M}_k^{2+}$.
% To analyse this scenario, we start considering episodes with a non-sufficient level of exploration (\ie $t_k < C(k) = \wt{\mathcal{O}}(D_c^2 S^3A)$), for which \tucrl suffers linear regret.
% Since the overall number of times this event happens is small, the contribute to the cumulative regret is polylogarithmic: $\sum_{k=1}^m \Delta_k \cdot \mathbbm{1}\lbrace t_k < C(k) \rbrace = \mathcal{O}(\rmaxbound D_c^2S^3A\ln^2\left(2SAT/\delta\right))$.
In the case $t_k \geq C(k)$, 
%we can identifies the possible scenarios (see App.~\ref{app:regret.Minset}).
we are able to prove that the solution found by EVI is \textbf{optimistic} for any $\mathcal{M}_k^\diamond$. The following lemma helps to identified the possible cases (see App.~\ref{app:regret.Minset}).
\begin{lemma}
        Let episode $k$ be such that $M^* \in \mathcal{M}^1_k$, $\calStrans_k\neq \emptyset$ and $t_k \geq C(k)$. 
        Then, either $\calStrans_k = \calStrans$ (case I) or there exists a state-action pair $(s,a) \in \calScom_k \times \A$ for which transitions to $\calStrans_k$ are allowed, \ie $N_k^{\pm}(s,a) \leq \sqrt{\sfrac{t_k}{SA}}$ (case II).
\end{lemma}
%As a consequence, either $\calStrans_k = \calStrans$ or there exists a state-action pair $(s,a) \in \calScom_k \times \A$ for which transitions to $\calStrans_k$ are allowed (\ie $N_k^{\pm}(s,a) \leq \sqrt{t_k/(SA)}$). For these two cases, it is possible to prove that the solution to problem~\ref{eq:tucrl.optimization} returned by EVI is \emph{optimistic}.
We start noticing that when $\calStrans_k = \emptyset$, the true MDP $M^* \in \mathcal{M}_k^1 = \mathcal{M}_k^2 = \mathcal{M}_k^\diamond$ w.h.p.
Similarly, if $\calStrans_k = \calStrans$ then $M^* \in \mathcal{M}_k^{2+} = \mathcal{M}_k^\diamond$ w.h.p., since \tucrl only truncates transitions that are already not available in $M^*$.
In both cases,  we can use the same arguments in~\citep{Jaksch10} to prove optimism.
Finally, note that in \emph{case II} the gain of any state $s' \in \calStrans_k$ is $\rmaxbound$ and, since there exists a path from $\calScom_k$ to $\calStrans_k$, the gain of the solution returned by EVI is $\rmaxbound$ (\ie optimistic).

%We report a sketch of the proof. \emph{I)} if $\calStrans_k = \calStrans$ then $M^* \in \mathcal{M}_k^{2+}$ and optimism can be proved as in~\citep[][Sec. 4.3 \& Thm. 7]{Jaksch10}.
%Note that $\mathcal{M}_k^{2+}$ is such that transitions to any $s' \in \calStrans_k$ are forbidden from any state-action pair $(s,a) \in (\calScom_k=\calScom) \times \A$ and this is true (by definition) in $M^*$ (\ie $p(s'|s,a) = \wt{p}(s'|s,a) = 0$). 
%For $(s,a,s') \notin \calScom_k \times \A \times \calStrans_k$, $p(s'|s,a) \in B_{p,k}^{1}(s,a,s') = B_{p,k}^{2}(s,a,s')$, then $p(\cdot|s,a) \in B_{p,k}^{2+}(s,a)$. 
%\emph{II)} noticing that $B_{r,k}^{2+}$ and $B_{p,k}^{2+}$ are such that there exists an MDP $M' \in \mathcal{M}_k^{2+}$ such that any $s' \in \calStrans_k$ is an absorbing state with reward $\rmaxbound$ and all the states $s \in \calScom_k$ are transient states (recall there is a path from $\calScom_k$ to $\calStrans_k$). It is possible to create such an MDP $M'$ since in $\calStrans_k$ the uncertainty is maximal (see App.~\ref{app:regret.Minset} for details). Thus, the gain of $M'$ is $\rmaxbound$. 
%As a consequence, in both cases $\wt{g}_k \geq g^*_{M^*} - \frac{\rmaxbound}{\sqrt{t_k}}$ and by denoting $\wt{\Delta}_k := \sum_{s,a} \nu_k(s,a) (\wt{g}_k - \wt{r}_k(s,a))$, we can further decompose the regret in episode $k$ as:
%\[
%\Delta_k \leq \wt{\Delta}_k + 2\sum_{s,a}\nu_k(s,a) \beta_{r,k}^{sa} + \rmaxbound \sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}}
%\]

Similarly to \ucrl, by exploiting the optimism and the optimality equation, we further decompose the regret at episode $k$.
We start focusing on the state-action pairs such that $\mathbbm{1}\{N_k^{\pm}(s,a) > \sqrt{\sfrac{t_k}{SA}}\} := \mathbbm{1}_k(s,a)$.
Lem.~\ref{lem:sum.bad.states} will show that the contribute to the cumulative regret is ``small'' in the case the reverse inequality holds.
In this case $\mathbbm{1}_k(s,a)$, the critical step is \textbf{bounding} the term involving \textbf{the optimistic vector} $\wt{h}_k$ computed by EVI (see Sec 4.3.2 in~\citep{Jaksch10} and App. F.6 in~\citep{fruit2018constrained}):
\begin{align*}
        \nu_k(\wt{P}_k -I)\wt{h}_k &= \sum_{s\in \wb{\calS}_k} \nu_k(s,\wt{\pi}_k(s)) \left(\sum_{s'\in \wb{\calS}_k}\wt{p}_k(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s) \right)
\end{align*}
where $w_k$ is a linear transformation of $\wt{h}_k$. 
Using Holder inequality the sum can be decomposed into the $\ell_1$-norm of the transition probabilities (that can be bounded using a concentration argument) and $sp_{\wb{\calS}_k}\{w_k\}$.
% The latter is the critical term since the $\ell_1$-norm can be bounded using concentration arguments.
% While the former can be bounded using a concentration argument, the span needs to be carefully handled.
In \ucrl, $\wb{\calS}_k = \calS$ and $\SP{w_k} \leq D$~\citep[][Sec. 4.3]{Jaksch10}.
Unfortunately, this results is uninformative when $M^*$ is weakly communicating.
However, using the new stopping condition, the truncation performed by $\mathcal{M}_k^{2+}$ and the condition $\mathbbm{1}_k(s,a)$, we can show that  $\wb{\calS}_k = \calScom_k$ in \tucrl 
and, since $w_k := \wt{h}_k - \min_{s\in\calScom_k}\{\wt{h}_k\}$, 
$sp_{\calScom_k}\{w_k\} = \max_{s\in\calScom_k}\{w_k\}$ is bounded by the diameter of the communicating part of $M^*$ (see App.~\ref{app:regret.Minset}).
We first introduce the following useful lemma (see App.~\ref{app:shortestpath} for details).
\begin{lemma}\label{L:sp.bias_difference}
            For any pair $(s,\wb{s}) \in \calS \times \calScom_k$,
            $\tau_{\mathcal{M}_k^{1+}}(s \to \wb{s}) = \tau_{\mathcal{M}_k^{2+}}(s \to \wb{s})$.
            Moreover, EVI on $\mathcal{M}_k^{2+}$ is such that (starting from the vector $\boldsymbol{0}$): $\wt{h}_k(s') - \wt{h}_k(s) \leq \rmaxbound \cdot \tau_{\mathcal{M}_k^{2+}}(s \to s')$, $\forall s,s' \in \calS$.
\end{lemma}
Since $M^* \in \mathcal{M}_k^{1+}$,  for all $s, s' \in \calScom_k$, $\tau_{\mathcal{M}_k^{1+}}(s \to s') \leq D_c$. Then, as a consequence of Lem.~\ref{L:sp.bias_difference}, for all $s,s' \in \calScom_k$,   $w_k(s) - w_k(s') =\wt{h}_k(s) - \wt{h}_k(s') \leq \rmaxbound D_c$.
We can now focus on the reverse inequality. In this case \tucrl suffers the maximum per-step regret $\rmaxbound$ but the number of times this event happen is ``small'' (see App.~\ref{sec:poorly.visited.states} for details):
\begin{lemma}\label{lem:sum.bad.states}
 For any $T \geq 1$ and any sequence of states and actions $\lbrace s_1, a_1, \dots \dots s_T, a_T \rbrace$ we have: 
\begin{align*}
        \sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^{\pm}(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace 
        &\leq
        \sum_{t=1}^{T}\mathbbm{1}\left\{ \max \lbrace 1, N_{k_t}(s_t,a_t)-1 \rbrace\leq \sqrt{\sfrac{t}{SA}} \right\} \\ % := D_T
        &\leq 2\sqrt{SAT} + 2SA
\end{align*}
%and $D_T \leq 2\sqrt{SAT} +2SA$.
\end{lemma}



%%% The critical term is:
%%% \begin{align*}
%%%         \nu_k'(\wt{P}_k -I)\wt{h}_k &= \sum_{s\in \calScom_k} \nu_k(s,\wt{\pi}_k(s))\mathbbm{1}_{k}(s,\wt{\pi}_k(s)) \left(\sum_{s'\in \calScom_k}\wt{p}_k(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s) \right)\\
%%%                        &\leq \left\|\wt{p}_k(\cdot|s,\wt{\pi}_k(s)) - p(\cdot|s,\wt{\pi}_k(s)) \right\|_1 \max_{s' \in \calScom_k} \lbrace w_k(s')\rbrace
%%% +\nu_k'(P_k -I)h_k
%%% \end{align*}
%%% where $\wt{h}_k$ is the vector computed by EVI and $w_k := \wt{h}_k - \min_{s\in\calScom_k} \{\wt{h}_k(s)\}$. Note that we have exploited the new \tucrl stopping condition 
%%% % ($\nu_k(s,\wt{\pi}_k(s)) = 0, \forall s \in \calStrans_k$)
%%% and the truncation performed by $\mathcal{M}_k^{2+}$
%%% %(if $\mathbbm{1}_k(s,\wt{\pi}_k(s)) =1$, then $\wt{p}(s'|s,\wt{\pi}_k(s))=0$ by construction for any $s' \in \calStrans_k$)
%%% to reduce the sum over states in $\calScom_k$.
%%% \citet{Jaksch10} showed that $\|w_k\|_{\infty} < D$ but $D=\infty$ if the true MDP $M^*$ is weakly communicating.
%%% By exploiting the structure of $\mathcal{M}_k^{2+}$ and the reduction to $\calScom_k$, we can show that $\max_{s \in \calScom_k} \{w_k\}$ is upper bounded by the diameter of the \emph{communicating} part of $M^*$. 
%%% We first introduce the following useful lemma (see App.~\ref{} for details).
%%% %% \begin{lemma}
%%% %%         The vectors $\wt{h}_k$ and $w_k$ are such that,
%%% %%             $\forall s,s' \in \calScom_k$,
%%% %% $w_k(s) - w_k(s') \leq \rmaxbound D_c$
%%% %% \end{lemma}
%%% \begin{lemma}\label{L:sp.bias_difference}
%%%             For any pair $(s,\wb{s}) \in \calS \times \calScom_k$,
%%%             $\tau_{\mathcal{M}_k^{1+}}(s \to \wb{s}) = \tau_{\mathcal{M}_k^{2+}}(s \to \wb{s})$.
%%%             Moreover, EVI on $\mathcal{M}_k^{2+}$ is such that (starting from $0$ vector): $\wt{h}_k(s) - \wt{h}_k(s') \leq \rmaxbound \cdot \tau_{\mathcal{M}_k^{2+}}(s \to s')$, $\forall s,s' \in \calS$.
%%% \end{lemma}
%%% Since $M^* \in \mathcal{M}_k^{1+}$,  for all $s, s' \in \calScom_k$, $\tau_{\mathcal{M}_k^{1+}}(s \to s') \leq D_c$. Then, as a consequence of Lem.~\ref{L:sp.bias_difference}, for all $s,s' \in \calScom_k$,   $w_k(s) - w_k(s') =\wt{h}_k(s) - \wt{h}_k(s') \leq \rmaxbound D_c$.
%%% %% The proof leverages on the fact that for any pair $(s,\wb{s}) \in \calS \times \calScom_k$,
%%% %%              $\tau_{\mathcal{M}_k^{1+}}(s \to \wb{s}) = \tau_{\mathcal{M}_k^{2+}}(s \to \wb{s})$.
%%% %%              and, for all $s,s' \in \calScom_k$,   $w_k(s) - w_k(s') =\wt{h}_k(s) - \wt{h}_k(s') \leq \rmaxbound D_c$ (see App.~\ref{}).
%%% %% Finally, since $M^* \in \mathcal{M}_k^{1+}$,  for all $s, s' \in \calScom_k$, $\tau_{\mathcal{M}_k^{1+}}(s \to s') \leq D_c$.




==> sec_exploration.tex <==
% !TEX root = tucrl.tex

\section{Optimistic Exploration-Exploitation}\label{sec:exploration}
Since our proposed algorithm \tucrl (Sec.~\ref{sec:tucrl}) is a variant of \ucrl, we first recall their common structure summarized in Fig.~\ref{fig:ucrl.constrained}.
%
\begin{figure}[t]
\renewcommand\figurename{\small Figure}
\begin{minipage}{\columnwidth}
\bookboxx{
\textbf{Input:} Confidence $\delta \in ]0,1[$, $r_{\max}$, $\calS$, $\A$, a constant $c \geq 0$

\noindent \textbf{Initialization:} Set $N_1(s,a) = 0$ for any $(s,a) \in \calS \times \A$, $t = 1$ and observe $s_1$.

\noindent \textbf{For} episodes $k=1, 2, ...$ \textbf{do}

\begin{enumerate}[leftmargin=4mm,itemsep=0mm]
\item Set $t_k = t$ and episode counters $\nu_k (s,a) = 0$

\item Compute estimates $\wh{p}_k(s' | s,a)$, $\wh{r}_k(s,a)$ and a confidence set~$\mathcal{M}_k$ (\ucrl, \regalc), resp.~$\mathcal{M}_k^\diamond$ (\tucrl)
%$\wt{\mathcal{M}}_k^\ddagger$ (based on Thm.~\ref{def:augmented.perturbed.mdp} with $\eta = 1/\sqrt{t_k}$)

\item
% Compute (an approximation of) the optimal policy $\widetilde{\pi}_k$ and the optimistic MDP $\widetilde{M}_k$, that is,
% $$(\wt{M}^*_k, \wt\pi^*_k ) \in \argmax_{M\in\mathcal{M}_k, \pi} g^\pi_M.$$
Compute an $\rmaxbound/\sqrt{t_k}$-approximation $\widetilde{\pi}_k$ of the solution of Eq.~\ref{eq:ucrl.optimization} (\ucrl), resp. Eq.~\ref{eq:optimistic.policy.regalc} (\regalc), resp. Eq.~\ref{eq:tucrl.optimization} (\tucrl)

%\item Use \regopt to compute an $1/\sqrt{t_k}$-approximation $\widetilde{\pi}_k$ of the solution of Eq.~\ref{eq:optimistic.policy.relaxedregalc} where $\mathcal{M}_k$ is replaced by $\mathcal{M}_k^{\ddagger}$ 
%
\item Sample action $a_t \sim \pi_k(\cdot|s_t)$

\item \textbf{While} 
%        $\nu_k(s_t,a_t) \leq \max\{1, N_k(s_t,a_t)\}$ 
        \textit{ stopping\_condition }
        \textbf{do}
%
\begin{enumerate}[leftmargin=4mm,itemsep=-1mm]
        \item Execute $a_t$, obtain reward $r_{t}$, and observe $s_{t+1}$
        \item Set $\nu_k (s_t,a_t) \pluseq 1$ 
        \item Sample action $a_{t+1} \sim \wt{\pi}_k(\cdot|s_{t+1})$ and set $t \pluseq 1$
\end{enumerate}

\item Set $N_{k+1}(s,a) = N_{k}(s,a)+ \nu_k(s,a)$ \tikz[baseline]{\node[anchor=base](alg_lastline){};}
\end{enumerate}
}
\caption{\small The general structure of optimistic algorithms for RL.}
\label{fig:ucrl.constrained}
\begin{tikzpicture}[overlay,font=\small]
        \draw[anchor=south west, draw=black] ($(alg_lastline) + (2cm,-0.2cm)$) rectangle ($(alg_lastline) + (8cm, 2.5cm)$);
        \coordinate (A) at ($(alg_lastline) + (2.3cm, 2.1cm)$);
        \node[anchor=west] at (A) {$\triangleright$~\emph{stopping\_condition} (\ucrl, \regalc)};
        \node[anchor=west] at ($(A)+(0.3cm,-.5cm)$) {$\nu_k(s_t,a_t) \leq \max\{1, N_k(s_t,a_t)$};
        % TUCRL
        \node[anchor=west] (TUCRL_stop) at ($(A)+(0, -1.cm)$) {$\triangleright$~\emph{stopping\_condition} (\tucrl)};
        \node[anchor=west] at ($(A)+(0.3cm,-1.4cm)$) {$t_k == t$ \textbf{or} $\Big( \sum_{a \in \A_{s_t}} N_k(s_t,a) > 0$ };
        \node[anchor=west] at ($(A)+(0.3cm,-2.cm)$) { \textbf{ and }$\nu_k(s_t,a_t) \leq \max\{1, N_k(s_t,a_t)\} \Big)$};
\end{tikzpicture}
\end{minipage}
\end{figure}


\ucrl is an algorithm designed to balance the trade-off between exploration and exploitation in communicating MDPs, \ie when $\calStrans = \emptyset$.
\ucrl proceeds through episodes $k=1,2\dots$ At the beginning of each episode $k$, \ucrl computes a set of plausible MDPs defined as
\begin{equation}
        \label{eq:plausible.mdps}
        \begin{aligned}
                \mathcal M_k^1 = \big\{ M = \langle \calS, \A, \wt{r}, \wt{p}\rangle \;:\; &\forall (s,a)\in \calS \times \A,~\wt{r}(s,a) \in B_{r,k}^1(s,a),\\
                                                                                           &\wt{p}(s'|s,a) \in B_{p,k}^1(s,a,s'),~ \wt{p}(\cdot|s,a) \in \mathcal{C}
                \big\}
        \end{aligned}
\end{equation}
where $\mathcal{C} = \{p \in \mathbb{R}^S | \forall s,~p(s) \geq 0 \wedge \sum_{s} p(s) = 1\}$ is the $(S-1)$-simplex, $B_{r,k}^1$ and $B_{p,k}^1$ are high-probability confidence intervals on the rewards and transition probabilities of the true MDP $M^*$, which guarantees that $M^* \in \mathcal{M}_k^1$ w.h.p.
In this paper we use confidence intervals constructed using the empirical Bernstein's inequality~\citep{audibert2007tuning,Maurer2009empirical}
\begin{align*}
\beta_{r,k}^{sa}
:=
         \sqrt{\frac{14 
                         \wh{\sigma}_{r,k}^2(s,a)
%        \ln(2 SA t_k/\delta)
                        b_{k,\delta}
                }{
%        \max\lbrace 1, N_k(s,a)\rbrace
        N^{+}_k(s,a)
}} + \frac{\frac{49}{3}
%                 \alpha_r 
\rmaxbound
%        \ln(2 SA t_k/\delta)
        b_{k,\delta}
        }{
        N^{\pm}_k(s,a)
%        \max\lbrace 1, N_k(s,a)-1 \rbrace
}
, \qquad
\beta_{p,k}^{sas'}
:= 
\sqrt{\frac{14 \wh{\sigma}_{p,k}^2(s'|s,a) 
%        \ln(2 SA t_k/\delta)
                        b_{k,\delta}
                }{
%        \max\lbrace 1, N_k(s,a)\rbrace
        N^{+}_k(s,a)
}
} +\frac{\frac{49}{3}
%                 \alpha_p 
%        \ln(2 SA t_k/\delta)
        b_{k,\delta}
        }{
        N^{\pm}_k(s,a)
%        \max\lbrace 1,N_k(s,a)-1 \rbrace
}
\end{align*}
where $N_k(s,a)$ is the number of visits in $(s, a)$ before episode $k$, 
$N^{+}_k(s,a) := \max\lbrace 1, N_k(s,a) \rbrace$, 
$N^{\pm}_k(s,a) := \max\lbrace 1, N_k(s,a)-1 \rbrace$, 
$\wh{\sigma}_{r,k}^2(s,a)$ and $\wh{\sigma}_{p,k}^2(s'|s,a)$ are the empirical variances of $r(s,a)$ and ${p}(s'|s,a)$ %respectively 
% (formally defined in eqn.~\eqref{eqn:def_empirical_variance} of App.~\ref{app:regret.reg.ucrl}) 
and $b_{k,\delta} = \ln(2 SA t_k/\delta)$.
%
Given the empirical averages $\wh{r}_k(s,a)$ and $\wh{p}_k(s'|s,a)$ of rewards and transitions, we define $\mathcal{M}_k^1$ by $B_{r,k}^1(s,a) := [\wh{r}_k(s,a) - \beta_{r,k}^{sa}, \wh{r}_k(s,a) + \beta_{r,k}^{sa}] \cap [0, \rmaxbound]$ and $B_{p,k}^1(s,a,s') := [\wh{p}_k(s'|s,a) - \beta_{p,k}^{sas'},\wh{p}_k(s'|s,a) + \beta_{p,k}^{sas'}] \cap [0,1]$.

Once $\mathcal{M}_k^1$ has been computed, \ucrl finds an approximate solution $(\wt{M}_k^*,\wt\pi_k^*)$ to the problem:
%
\begin{align}\label{eq:ucrl.optimization}
( \wt{M}^*_k, \wt\pi^*_k ) \in \argmax_{M\in\mathcal{M}_k, \pi\in\SD(M)} g^\pi_M.
\end{align}
%
Since $M^* \in \mathcal{M}_k^1$ w.h.p., then ${g}^*_{\wt{M}_k} \geq  {g}^*_{M^*}$.
As noticed by~\citet{Jaksch10}, problem~\eqref{eq:ucrl.optimization} is equivalent to finding $\wt{\mu}^* \in \argmax_{\mu \in \SD(\wt{\mathcal{M}}_k)} \big\lbrace g^\mu_{\wt{\mathcal{M}}_k} \big\rbrace$ where $\wt{\mathcal{M}}_k$ is the \emph{extended} MDP (sometimes called \emph{bounded-parameter} MDP) implicitly defined by $\mathcal{M}_k^1$. More precisely, in $\wt{\mathcal{M}}_k$ the (finite) action space $\A$ is ``extended'' to a compact action space $\wt{\A}_k$ by considering every possible value of the confidence intervals $B_{r,k}^1(s,a)$ and $B_{p,k}^1(s,a,s')$ as fictitious actions. The equivalence between the two problems comes from the fact that for each $\wt{\mu} \in \SD(\wt{\mathcal{M}}_k)$ there exists a pair ($\wt{M}, \wt{\pi}$) such that the policies $\wt{\pi}$ and $\wt{\mu}$ induce the same Markov Reward Process (MRP) on respectively $\wt{M}$ and $\wt{\mathcal{M}}_k$, and conversely. Consequently, \eqref{eq:ucrl.optimization} can be solved by running so-called \textit{extended} value iteration (\evi): starting from an initial vector $u_0 =0$, \evi recursively computes
%
\begin{align}\label{eq:evi}
        u_{n+1}(s) \!=\! \max_{a \in \A_s} \left\{ \max_{\wt{r} \in B_{r,k}^1(s,a)}\wt{r} + \max_{\wt{p} \in B_{p,k}(s,a,\cdot)} \left\{ \wt{p}^\transp u_n \right\} \right\} \!=\! \wt{L}_{\mathcal{M}_k^1} u_n(s),
\end{align}
where $\wt{L}_{\mathcal{M}_k^1}$ is the \textit{optimistic} optimal Bellman operator associated to $\wt{\mathcal{M}}_k$. 
If \evi is stopped when $\SP{u_{n+1}-u_n} \leq \varepsilon_k$, then the greedy policy $\wt{\mu}_{k}$ \wrt $u_{n}$ is guaranteed to be $\varepsilon_k$-optimal, \ie $g^{\wt{\mu}_{k}}_{\wt{\mathcal{M}}_k} \geq {g}^*_{\wt{\mathcal{M}}_k} - \varepsilon_k \geq {g}^*_{M^*} - \varepsilon_k $. Therefore, the policy $\wt{\pi}_k$ associated to $\wt{\mu}_{k}$ is an \emph{optimistic} $\varepsilon_k$\emph{-optimal} policy, and \ucrl executes $\wt{\pi}_k$ until the end of episode $k$.





==> sec_limits.tex <==
% !TEX root = tucrl.tex

\section{Successes and limitations of optimistic approaches in RL}\label{sec:limits}
% \begin{itemize}
%         \item UCRL unable to learn in weakly communicating MDPs (only when $\calStrans = \emptyset$)
%         \item $\implies$ REGAL $\implies$ SCAL
%         \item example motivating $\sqrt{T}$
%         \item misspecified states
% \end{itemize}

In this section we analyse the \emph{exploration-exploitation trade-off} when the learning agent evolves in a \emph{weakly-communicating} MDP ($D\leq+\infty$). We first give a brief overview of existing regret guarantees for \emph{communicating} MDPs (the learning agent exploits the prior knowledge $D<+\infty$) and weakly-communicating MDPs with prior knowledge on the optimal bias span $\SP{h^*}$ (Sec.~\ref{sec:regret_prior}). We then present a \emph{no free lunch} theorem when $\SP{h^*}$ is unknown (Sec.~\ref{sec:no_free_lunch}). Finally, we give new insights on \emph{regularised} optimistic approaches \citep[\regal]{Bartlett2009regal} (Sec.~\ref{sec:regal}).
% Our goal is to show on a simple example (Ex.~\ref{ex:weakly_communicating}) that learning is \emph{intrinsically} more difficult in this case.

\subsection{Regret guarantees with prior knowledge: state-of-the-art}\label{sec:regret_prior}
We first recall that the expected regret $\mathbbm{E}[\Delta(\ucrl,M,T)]$ of $\ucrl$ (with input parameter $\delta =1/3T$) after $T\geq 1$ time steps and for any finite MDP $M$ can be bounded in several ways: 
\begin{align}\label{eqn:regret_bound_ucrl}
 \hspace{-0.1in}\mathbbm{E}[\Delta(\ucrl,M,T)] \leq \begin{cases}
                                    \rmaxbound T~~\text{(by definition)}\\
                                    C_1 \cdot\rmaxbound DS \sqrt{AT\ln(3T^2)} +\frac{1}{3} ~\text{\citep[Theorem 2]{Jaksch10}}\\
                                    C_2 \cdot \rmaxbound \frac{D^2 S^2 A}{\gamma} \ln(T) + C_3(M)~\text{\citep[Theorem 4]{Jaksch10}}
                                   \end{cases}
\end{align}
where $C_1:= 34$ and $C_2:=34^2$ are numerical constants independent of the MDP $M$ considered, $\gamma=g^*_M - \max_{s,\pi}\{g^\pi_M(s):~ g^\pi_M(s) < g^*_M \} $ and $C_3(M):= O(\max_{\pi: \pi(s)=a} T_{\pi})$
% \[C_3(M):=1+\sum_{s,a} \left\lceil 1 + \log_2\left( \max_{\pi: \pi(s)=a} T_{\pi} \right)\right\rceil \cdot\max_{\pi: \pi(s)=a} T_{\pi}\] 
% with $T_\pi$ the smallest natural number such that for all $T\geq T_\pi$, the expected average reward after $T$ steps is $g/2$-close to the average reward of $\pi$. 
with $T_\pi$ a measure of the ``mixing time'' of policy $\pi$ \citep[Theorem 4]{Jaksch10}. The three different bounds lead to three different \emph{``regimes''} for the function $T \longmapsto \mathbbm{E}[\Delta(\ucrl,M,T)]$ as is illustrated on Fig.~\ref{fig:ucrl.regimes_example.misspec}\emph{(left)}:
% ~\ref{fig:regret_regimes}:
% \begin{enumerate}
 1) for ${T}_M^\dagger \geq T \geq 0$, the expected regret is linear in $T$,
 2) for ${T}_M^* \geq T \geq {T}_M^\dagger$ the expected regret grows as $\sqrt{T}$,
 3) finally for $T\geq {T}_M^*$, the increase in regret is only logarithmic in $T$.
% \end{enumerate}
% For ${T}_M^\dagger \geq T \geq 0$, the expected regret is linear in $T$, while for ${T}_M^* \geq T \geq {T}_M^\dagger$ the expected regret grows as $\sqrt{T}$ and finally for $T\geq {T}_M^*$, the increase in regret is only logarithmic in $T$. 
As a direct consequence of \eqref{eqn:regret_bound_ucrl}, ${T}_M^\dagger$ is bounded by ${O}(D^2 S^2 A)$ which is polynomial in the parameters of the MDP. ${T}_M^*$ depends (linearly) on $\max_{\pi: \pi(s)=a} T_{\pi}$ and  $1/\gamma$ which can also be considered as parameters of the MDP and so ${T}_M^*$ is also polynomial in the parameters of $M$. It is easy to verify theoretically and empirically that when the MDP is not communicating (\ie when $D = +\infty$), the regret of \ucrl grows linearly with $T$ (\ie ${T}_M^\dagger = {T}_M^* = +\infty$). In this case, \ucrl never \emph{learns} (refer to Sec.~\ref{sec:regal} for a more detailed explanation). The first attempt in the literature to overcome this major limitation was proposed by \citet{Bartlett2009regal} who derived three ``pseudo-algorithms''\footnote{None of these ``algorithms'' is actually implementable for various reasons, see \citep{fruit2018constrained} for further details.}: \regal, \regalc and \regald. We postpone the discussion about \regal and \regald to Sec.~\ref{sec:regal} and restrict attention to \regalc for now. The idea of \regalc is to incorporate prior knowledge into \ucrl to not only be able to learn when $D = +\infty$, but also improve the regret when $D <+\infty$. More precisely, \regalc takes as input a finite upper-bound $H<+\infty$ on the optimal bias span of the true MDP $\SP{h^*}$\footnote{By definition, $\SP{h^*}<+\infty$ for any MDP (even if $D = +\infty$).}. As a result, the regret guarantees of \regalc are identical to those of \ucrl with $\rmaxbound D$ replaced by $\min\{H,\rmaxbound D\}$. \citet[Theorem 4]{Bartlett2009regal} also showed that $\SP{h^*} \leq \rmaxbound D$ and in many MDPs $\SP{h^*}$ is actually much smaller than $\rmaxbound D$. Therefore, if $H$ is close enough to $\SP{h^*}$, the improvement of \regalc over \ucrl is potentially huge. Unfortunately, \regalc involves solving a complex optimisation problem that is probably intractable. Recently, \citet{fruit2018constrained} relaxed the optimisation problem solved by \regalc and derived an efficient algorithm -- \scal -- that enjoys the same theoretical guarantees as \regalc. Although they only provide an analogue of Theorem 2 of \citet{Jaksch10} (Theorem 12) \ie a $O(\sqrt{T})$ regret bound with $D$ replaced by $H$, it seems straightforward to extend their result to a $O(\ln({T}))$ regret bound (analogue of Theorem 4 of \citet{Jaksch10} with $D$ replaced by $H$). It is still an opened question whether the same guarantees can be derived when no upper-bound on $\SP{h^*}$ is available. We will not provide an answer to this question but we will show in the next section that when $D = +\infty$ and $\SP{h^*}$ is unknown, any \emph{efficient} learning algorithm must be such that ${T}_M^* =+\infty$.
% {\color{blue} To the best of our knowledge, the current belief in the literature so far is that it is possible to derive similar guarantees when the MDP is weakly communicating using a different algorithm. Such an algorithm should then scale with a different quantity than $D$. The research direction investigated so far was to replace $D$ by the span of the optimal bias $\SP{h^*}$ which is always finite. The span of the optimal bias is very appealing as it always satisfies $\SP{h^*}\leq \rmaxbound D$ and it is very easy to interpret: it bounds the total amount of regret incurred when deviating from the optimal policy in just one step (\ie making one mistake and then applying the optimal policy). \citet{fruit2018constrained} showed that when the value $\SP{h^*}$ is known to the learning agent, this is indeed possible. However, this is still an opened question whether the same guarantees can be derived when $\SP{h^*}$ is unknown.  We think that this is probably not a very desirable property for an efficient learning algorithm meaning that any ``good'' algorithm should give up on having a logarithmic increase of the regret for $T\geq {T}_M^*$ (\ie ${T}_M^* < + \infty$). In the next section we will present an algorithm that achieves $\sqrt{T}$ regret for any $T \geq {T}_M^\dagger$ and for which ${T}_M^* = + \infty$ whenever $D = +\infty$.}
In this paper, we focus on \emph{frequentist} regret guarantees and algorithms using OFU. There is also an extensive literature on Bayesian methods for RL (Posterior sampling) with guarantees on the expected Bayesian regret usually. We briefly discuss state-of-the-art approaches

%% \begin{figure}[h]
%% \centering
%%  \begin{tikzpicture}[domain=0:4]
%%     \draw[very thin,color=gray] (-0.1,-0.1) (10,3.9);
%%     \draw[->] (-0.2,0) -- (10,0) node[right] {$T$};
%%     \draw[->] (0,-0.2) -- (0,4.2) node[above] {$\mathbb{E}[\Delta(\ucrl,T,M)]$};
%%     
%%     \draw[scale=1,domain=0:5,smooth,variable=\x,green,samples=100] plot ({\x},{0.8*\x});
%%     \draw[scale=1,domain=0:10,smooth,variable=\x,blue,samples=400] plot ({\x},{1.3*\x^(0.5)});
%%     \draw[scale=1,domain=0.03:10,smooth,variable=\x,red,samples=100] plot ({\x},{2.1+0.65*ln(\x)});
%%     
%%     \draw[scale=1,domain=0:2.64,smooth,variable=\x,black,samples=100, line width=1.75pt] plot ({\x},{0.8*\x});
%%     \draw[scale=1,domain=2.64:6.49,smooth,variable=\x,black,samples=100, line width=1.75pt] plot ({\x},{1.3*\x^(0.5)});
%%     \draw[scale=1,domain=6.49:10,smooth,variable=\x,black,samples=100, line width=1.75pt] plot ({\x},{2.1+0.65*ln(\x)});
%%     
%%     \node () at (5.2,4.4){\color{green}$O(T)$};
%%     \node () at (8.4,4.4){\color{blue}$O(DS\sqrt{AT\ln(T)})$};
%%     \node () at (1.7,3.3){\color{red}$O\left(\frac{D^2 S^2 A}{\gamma} \ln(T)\right)$};
%%     
%%     \node (1) at (2.64,2.17){};
%%     \node (2) at (2.64,-0.1){};
%%     \node (3) at (6.49,3.4){};
%%     \node (4) at (6.49,-0.1){};
%%     
%%     \node () at (-0.2,-0.4){$0$};
%%     \node () at (2.64,-0.3){${T}_M^\dagger$};
%%     \node () at (6.49,-0.3){${T}_M^*$};
%%     
%%     \node (5) at (9,2.){Regret upper-bound};
%%     \node (6) at (9,3.6){};
%%     
%%     \draw[-,dashed, >=latex](1) to node[above]{} (2);
%%     \draw[-,dashed, >=latex](3) to node[above]{} (4);
%%     
%%     \draw[-,->] (5) to (6);
%% \end{tikzpicture}
%% \caption{Expected regret of $\ucrl$ (with known horizon $T$ given as input) as a function of $T$.}
%% \label{fig:regret_regimes}
%% \end{figure}

\subsection{No free lunch}\label{sec:no_free_lunch}

%% \begin{figure}[h]
%% \centering
%% \begin{subfigure}[b]{0.5\textwidth}
%%  \begin{tikzpicture}
%% \begin{scope}[scale=0.86]
%% 	\tikzset{VertexStyle/.style = {draw, 
%% 									shape          = circle,
%% 	                                text           = black,
%% 	                                inner sep      = 2pt,
%% 	                                outer sep      = 0pt,
%% 	                                minimum size   = 24 pt}}
%% 	\tikzset{VertexStyle2/.style = {shape          = circle,
%% 	                                text           = black,
%% 	                                inner sep      = 2pt,
%% 	                                outer sep      = 0pt,
%% 	                                minimum size   = 14 pt}}
%% 	\tikzset{Action/.style = {draw, 
%%                 					shape          = circle,
%% 	                                text           = black,
%% 	                                fill           = black,
%% 	                                inner sep      = 2pt,
%% 	                                outer sep      = 0pt}}
%% 	                                 
%%     % Node of the MDP
%% 	\node[VertexStyle,fill=gray](s0) at (0,0) {$ x $};
%% 	\node[Action](a0s0) at (.4,0.9){};
%% 	\node[Action](a1s0) at (.4,-.9){};
%% % 	\node[VertexStyle](s1) at (5,0){$s_1$};
%% % 	\node[Action](a0s1) at (1.5,0.){};
%% 	\node[VertexStyle](s2) at (5,0){$y$};
%% 	\node[Action](a0s2) at (4.,0){};
%% 	\node[Action](a1s2) at (6,0.){};
%%     
%% 	% Edges of the MDPsec:regal
%% 	\draw[->, >=latex, double, color=red](s0) to node[midway, right]{{ $b$}} (a0s0);
%% 	\draw[->, >=latex, double, color=red](s0) to node[midway, right]{{ $d$}} (a1s0);
%% 	\draw[->, >=latex](a0s0) to [out=45,in=120,looseness=0.8] node[above]{$\varepsilon$} (s2);
%% 	\draw[->, >=latex](a0s0) to [out=80,in=140,looseness=3] node[above]{$1-\varepsilon$} (s0);
%% 	\draw[->, >=latex](a1s0) to [out=-80,in=-140,looseness=3] node[above]{} (s0);
%% 	\draw[->, >=latex, double, color=red](s2) to node[midway, above]{{ $d$}} (a0s2);   
%% 	\draw[->, >=latex](a0s2) to [out=180, in=360, looseness=0.] node[above]{} (s0);
%% 	\draw[->, >=latex, double, color=red](s2) to node[midway, below]{{ $b$}} (a1s2);
%% 	\draw[->, >=latex](a1s2) to [out=-10, in=-85, looseness=3] (s2);
%% 
%%     % Define reward
%%     \node [right, xshift=0.2em, yshift=0.2em] at (a0s0) { $r=0$};
%%     \node [right, xshift=0.2em, yshift=-0.2em] at (a1s0) { $r=1/2$};
%%     \node [below, yshift=-0.2em] at (a0s2) { $r = 0$};
%%     \node [above, yshift=0.2em] at (a1s2) { $r =1$};  
%%     \end{scope}
%% \end{tikzpicture}
%% \caption{\label{fig:delta_pos}}
%% \end{subfigure}
%% \begin{subfigure}[b]{0.45\textwidth}
%% % \hspace{-.7in}
%% \begin{tikzpicture}
%% \begin{scope}[scale=0.86]
%% 	\tikzset{VertexStyle/.style = {draw, 
%% 									shape          = circle,
%% 	                                text           = black,
%% 	                                inner sep      = 2pt,
%% 	                                outer sep      = 0pt,
%% 	                                minimum size   = 24 pt}}
%% 	\tikzset{VertexStyle2/.style = {shape          = circle,
%% 	                                text           = black,
%% 	                                inner sep      = 2pt,
%% 	                                outer sep      = 0pt,
%% 	                                minimum size   = 14 pt}}
%% 	\tikzset{Action/.style = {draw, 
%%                 					shape          = circle,
%% 	                                text           = black,
%% 	                                fill           = black,
%% 	                                inner sep      = 2pt,
%% 	                                outer sep      = 0pt}}
%% 	                                 
%%     % Node of the MDP
%% 	\node[VertexStyle,fill=gray](s0) at (0,0) {$ x $};
%% 	\node[Action](a0s0) at (.4,0.9){};
%% 	\node[Action](a1s0) at (.4,-.9){};
%% % 	\node[VertexStyle](s1) at (5,0){$s_1$};
%% % 	\node[Action](a0s1) at (1.5,0.){};
%% 	\node[VertexStyle](s2) at (5,0){$y$};
%% 	\node[Action](a0s2) at (4.1,-0.5){};
%% 	\node[Action](a1s2) at (4.1,0.5){};
%%     
%% 	% Edges of the MDP
%% 	\draw[->, >=latex, double, color=red](s0) to node[midway, right]{{ $b$}} (a0s0);
%% 	\draw[->, >=latex, double, color=red](s0) to node[midway, right]{{ $d$}} (a1s0);
%% % 	\draw[->, >=latex](a0s0) to [out=45,in=120,looseness=0.8] node[above]{$\varepsilon$} (s2);
%% 	\draw[->, >=latex](a0s0) to [out=80,in=140,looseness=3] node[above]{} (s0);
%% 	\draw[->, >=latex](a1s0) to [out=-80,in=-140,looseness=3] node[above]{} (s0);
%% 	\draw[->, >=latex, double, color=red](s2) to node[midway, below]{{ $b$}} (a0s2);   
%% 	\draw[->, >=latex](a0s2) to [out=200, in=-20, looseness=0.8] node[above]{} (s0);
%% 	\draw[->, >=latex, double, color=red](s2) to node[midway, above]{{ $d$}} (a1s2);
%% 	\draw[->, >=latex](a1s2) to [out=160, in=20, looseness=0.8] (s0);
%% 
%%     % Define reward
%%     \node [right, xshift=0.2em, yshift=0.2em] at (a0s0) { $r=0$};
%%     \node [right, xshift=0.2em, yshift=-0.2em] at (a1s0) { $r=1/2$};
%%     \node [below, xshift=-0.5em,yshift=-0.2em] at (a0s2) { $r = 1$};
%%     \node [below, xshift=-0.5em,yshift=-0.2em] at (a1s2) { $r =0$};  
%%      \end{scope}
%% \end{tikzpicture}
%% \caption{\label{fig:delta_zero}}
%% \end{subfigure}
%% \caption{Toy example illustrating the difficulty of learning non-communicating MDPs. We represent a family of possible MDPs $\mathcal{M} = (M_\varepsilon)_{\varepsilon \in [0,1]}$ where the probability $\varepsilon$ to go from $x$ to $y$ lies in $[0,1]$. 
%% % \ref{fig:delta_pos} $\varepsilon >0$ and optimal gain $g^*_\varepsilon =1$ and \ref{fig:delta_zero} $\varepsilon =0$ and optimal gain $g^*_0 =1/2$.
%% }\label{fig:exploration_exploitation_misspecified}
%% \end{figure}

\input{sec_limits_pics}

\begin{example}\label{ex:weakly_communicating}
        We consider a family of weakly-communicating MDPs $\mathcal{M} = (M_\varepsilon)_{\varepsilon \in [0,1]}$ represented on Fig.~\ref{fig:ucrl.regimes_example.misspec}\emph{(right)}.
% ~\ref{fig:exploration_exploitation_misspecified}. 
 Every MDP instance in $\mathcal{M}$ is characterised by a specific value of $\varepsilon \in [0,1]$ which corresponds to the probability to go from $x$ to $y$. For $\varepsilon>0$ \ref{fig:delta_pos}, the optimal policy of $M_\varepsilon$ is such that $\pi^*(x) = b$ and the optimal gain is $g^*_\varepsilon = 1$ while for $\varepsilon=0$ \ref{fig:delta_zero} the optimal policy is such that $\pi^*(x) = d$ and the optimal gain is $g^*_0 = 1/2$. We assume that the learning agent knows that the true MDP $M^*$ belongs to $\mathcal{M}$ but does not know the value $\varepsilon^*$ associated to $M^*$ \ie $M^*=M_{\varepsilon^*} $ with $\varepsilon^* \in [0,1]$ \emph{completely} unknown. For simplicity, we may assume that all rewards are deterministic although this is not necessary. The agent starts in state $x$ (coloured in grey).
\end{example}

  Ex.~\ref{ex:weakly_communicating} can be seen as a multi-armed bandit problem with two ``arms'' -- $b$ and $d$ -- and an additional highly rewarding state $y$ that might or might not be reachable from $x$. In the classical stochastic multi-armed bandit setting the agent knows that $\varepsilon^* =0$ and \textsc{UCB} achieves near-optimal regret guarantees by applying the ``optimism in the face of uncertainty principle'' which consists in pulling the arm with highest optimistic reward at any time $t\geq 1$ \ie $ a_t\in\argmax_{a \in \{ b,d\}}\left\{ r(x,a) + O\left(\sqrt{{\ln(t/\delta)}/{N_t(x,a)}}\right) \right\}$ where $N_t(x,a)$ denotes the number of times ``arm'' $a$ was pulled up to time step $t$ ($t$ excluded). With this strategy we can easily show that at any time $t$, the gap in rewards between the optimal ``arm'' $a^*$ and the ``arm'' $a_t$ pulled at time $t$ is bounded as $\gamma_t := r(x,a^*)-r(x,a_t) = O\left(\sqrt{{\ln(t/\delta)}/{N_t(x,a_t)}}\right)$ (with probability at least $1-\delta$) even if $a^*$ is not known. With high probability, the loss incurred at every time step $t$ is controlled and since by definition $\mathbbm{E}[\Delta(T)] = \mathbbm{E}\left[\sum_{t=1}^{T}\gamma_t\right]$, it is then easy to derive regret bounds both in $O(\ln(T))$ and $O(\sqrt{T})$.
%   Exploiting this last inequality together with the fact that $ \Delta(T) \leq \min \left\{ \sum_{a \neq a^*}\gamma_a N_T(x,a)~, \gamma T \right\}$, it is possible to derive high probability bounds on the regret (both logarithmic and $O(\sqrt{T})$). 
  Similarly, in Ex.~\ref{ex:weakly_communicating} the value of $\varepsilon^*$ is unknown but can be bounded at any time $t$ by $O\left(\sqrt{{\ln(t/\delta)}/{N_t(x,b)}}\right)$ (with probability at least $1-\delta$). The quantity of interest in the general reinforcement learning setting is no longer the immediate reward $r$ like in the bandit case, but the long-term average reward (or gain) $g$\footnote{In the bandit setting, all transitions loop on the same (unique) state and so the immediate reward coincides with the gain.}. For $\varepsilon >0$ the optimal gain $g^*_\varepsilon$ is equal to $1$ no matter how small $\varepsilon$ is, while $g^*_0 =1/2$. As long as $y$ has not been visited, even for an arbitrarily large number of visits $N_t(x,b)$, the high confidence interval around $\varepsilon^*$ always contains $0$ and positive values implying that both alternatives $\varepsilon^* >0$ and $\varepsilon^* =0$ are equally plausible. Therefore, despite our knowledge on $\varepsilon^*$, it is not possible to bound the gap in average gain $\gamma_t := g^*-g(x,a_t) $ between the optimal ``arm'' and the optimistic ``arm'' $a_t \in \{b,d\}$ pulled at time $t$. Unlike in the bandit case, the number of visits in $(x,b)$ does not provide any useful information on how close $b$ is to the optimal action in average gain. Only a visit in state $y$ can provide such an information but this might never happen if $\varepsilon =0$ \ie if the MDP is not communicating. In Lem.~\ref{lem:weakly_communicating} wee formally prove that the exploration-exploitation dilemma is more challenging when $\mathcal{M}$ contains $M_0$.
  
%   (we call such a state ``misspecified'')
%  when the expected rewards of two potentially optimal arms are $\varepsilon$-close, the immediate regret incurred by an agent pulling the sub-optimal arm is at most $\varepsilon$. As a consequence, it is only necessary to identify the best arm up to an $\varepsilon$-accuracy with $\varepsilon$ small enough (typically $1/\sqrt{T}$) to guarantee a small regret. In our example, even though it might be arbitrarily hard to discriminate between two plausible MDPs $M_0$ and $M_\varepsilon$ when $\varepsilon$ is close enough to $0$, the difference in gain (often called ``gap'' in the bandit literature) is always $1/2 >> \varepsilon$ implying that any mistake might incur a big regret. 

% We now analyse Ex.~\ref{ex:weakly_communicating} in detail.        
\begin{lemma}\label{lem:weakly_communicating}
 Let $C_1, C_2,\alpha, \beta >0$ be positive real numbers and $f$ a function defined for all $\varepsilon \in ]0,1]$ by $f(\varepsilon) =  C_1 (1/\varepsilon)^{\alpha}$.
  There exists no learning algorithm $\mathfrak{A}_T$ (with known horizon $T$) satisfying both
  \vspace{-0.07in}
 \begin{enumerate}[leftmargin=*,nolistsep, topsep=0pt]
  \item for all $\varepsilon \in ]0,1]$, there exists ${T}_\varepsilon^\dagger \leq f(\varepsilon)$ such that $\mathbbm{E}[\Delta(\mathfrak{A}_T,M_\varepsilon,x,T)] < 1/6\cdot T$ for all $T \geq {T}_\varepsilon^\dagger$,
  \item and there exists ${T}_0^* < +\infty$ such that $\mathbbm{E}[\Delta(\mathfrak{A}_T,M_0,x,T)] \leq C_2 (\ln(T))^\beta$ for all $T \geq {T}_0^*$.
  \end{enumerate}
\end{lemma}

We will now discuss the implications of Lem.~\ref{lem:weakly_communicating}. All the MDPs in $\mathcal{M}$ share the same number of states $S=2$, number of actions $A=2$, and gap in average reward $\gamma=1/2$. As a result, any function of $S$, $A$ and $\gamma$ can be considered as constant in Ex.~\ref{ex:weakly_communicating}. For $\varepsilon >0$, the diameter coincides with the optimal bias span of the MDP and $D=\SP{h^*}=1/\varepsilon <+\infty$, while for $\varepsilon = 0$ the diameter is infinite $D = +\infty$ but $\SP{h^*} = 1/2 $. As we recalled in Sec.~\ref{sec:regret_prior}, both \scal and \ucrl satisfies property \emph{1.} of Lem.~\ref{lem:weakly_communicating} with $\alpha =2$ and $C_1 = O(S^2 A)$. Moreover, an analogue of property \emph{2.} also holds \ie there exists $C_2' = O({S^2A}/{\gamma})$ such that:

\emph{2'. $\forall \varepsilon \in ]0,1]$, $\exists {T}_\varepsilon^* < +\infty$ s.t. $\forall T \geq {T}_\varepsilon^*$, $\mathbbm{E}[\Delta(\ucrl/\scal,M_\varepsilon,x,T)] \leq C_2' (1/\varepsilon)^2 \ln(T)$.}

Finally, when $\varepsilon = 0$ and an input parameter $H \geq \SP{h^*_0} =1/2$ is used, \scal also satisfies \emph{2} (with $C_2$ scaling linearly with $H$). Nevertheless, \scal needs the knowledge of $H$ to achieve such performance, which amounts to knowing that either $\varepsilon^* =0$ or $\varepsilon^* \geq 1/H$ ($\varepsilon^*$ cannot be positive and arbitrarily small). On the other hand, Lem.~\ref{lem:weakly_communicating} shows that when the value of $\varepsilon^*$ is \emph{truly} unknown, there is \emph{no free lunch} \ie if the regret of the non-communicating MDP $M_0$ asymptotically grows as $O((\ln(T))^\beta)$, then there exist communicating MDPs with diameter $D$ that suffer a linear regret for at least $O\left(\exp\left(D^{1/\beta}\right)\right)$ time steps. In other words, the price to pay for an asymptotic logarithmic regret bound in non-communicating MDPs is an exponential cumulative loss for (some) communicating MDPs. Despite the simplicity of Ex.~\ref{ex:weakly_communicating}, to the best of our knowledge we are the first to formally state and prove such a result.

Although asymptotic guarantees are theoretically appealing, the main goal of RL is to be able to \emph{learn} using as few samples as possible. It seems therefore reasonable to expect that the regret of an \emph{efficient} RL algorithm should not -- if possible -- scale exponentially in the parameters of the MDP. As a consequence of Lem.~\ref{lem:weakly_communicating}, such an algorithm cannot achieve asymptotic logarithmic regret in non-communicating MDPs. In Sec.~\ref{sec:tucrl} we will introduce an algorithm -- \tucrl -- which achieves $O(\sqrt{T})$ regret for any weakly communicating MDP, and $O(\ln(T))$ only when the MDP is \emph{communicating} ($D <+\infty$). 
% In the next section we will present an algorithm that achieves $\sqrt{T}$ regret for any $T \geq {T}_M^\dagger$ and for which ${T}_M^* = + \infty$ whenever $D = +\infty$.

\subsection{Regularized optimistic RL (\regal)}\label{sec:regal}

We conclude Sec.~\ref{sec:limits} with a discussion on regularised optimistic approaches in RL, first introduced by \citet{Bartlett2009regal} for exploration-exploitation in weakly-communicating MDPs and then used in other contexts (see for example \citep{pmlr-v28-maillard13}). \ucrl works by episodes and at each episode plays a (stationary) gain-optimal policy $\wt{\pi}$ of the MDP $\wt{M}$ with highest optimal gain among all ``plausible'' MDPs. The set of plausible MDPs $\mathcal{M}$ is constructed using confidence intervals (see Sec.~\ref{sec:tucrl}) so as to ensure that with high probability, it contains the true unknown MDP $M^*$. When $M^* \in \mathcal{M}$, it is straightforward to show that $g_{\wt{M}}^* \geq g_{M^*}^*$ and so \ucrl is \emph{gain-optimistic}. Unfortunately when $M^*$ is non-communicating, some states will never be visited. $\mathcal{M}$ will then always contain an action that loops on these states with probability $1$ and reward $\rmaxbound$. As a consequence, \ucrl is way too optimistic ($g_{\wt{M}}^* =\rmaxbound$) and suffers linear regret. To avoid this problem, the intuition of \citet{Bartlett2009regal} was to penalise the optimism on $g^*$ by the optimal bias span $\SP{h^*}$ \ie find the MDP $\wt{M}'\in \mathcal{M}$ that maximises $g_{M}^* - \lambda \cdot \SP{h_{M}^*}$ where $\lambda\geq 0$ is a regularisation coefficient. The term $\SP{h^*}$ can be interpreted as a measure of the \emph{complexity} of the environment: the bigger $\SP{h^*}$, the more difficult it is to achieve the stationary reward $g^*$ by following the optimal policy. In \emph{supervised learning}, regularisation is often used to penalise the objective function by a measure of the complexity of the model so as to avoid \emph{overfitting}. It is thus reasonable to expect that \emph{over-optimism} in online RL can also be avoided through regularisation. The regret bound of \regal holds only when $\lambda$ is set to $\Theta (1/\sqrt{l_k})$ where $l_k$ is the length of the future episode. Unfortunately, an episode stops when the number of visits in a state-action pair $(s,a) \in \calS \times \mathcal{A}$ has doubled and it is not possible to predict the future sequence of states of a given policy for two reasons: 1) the true MDP $M^*$ is unknown and 2) what is observed is a random \emph{sampled} trajectory (as opposed to \emph{expected}). As a result, \regal is not \emph{implementable}. \citet{Bartlett2009regal} proposed an alternative algorithm -- \regald -- that leverages on the \emph{doubling trick} to guess the value of $l_k$ and proved a slightly worse regret bound than for \regal. Nevertheless, in Ex.~\ref{ex:weakly_communicating}, knowing the length of an episode (at least on expectation) seems to be equivalent to knowing $\varepsilon$ (or at least knowing whether $\varepsilon =0$ or $\varepsilon >0$ which is the main issue as discussed in Sec.~\ref{sec:no_free_lunch}). According to Lem.~\ref{lem:weakly_communicating}, this would imply that \regald does not admit any $O(\ln(T)^\beta)$ regret bound (for arbitrary $\beta>0$). Although such a bound is never proved by \citet{Bartlett2009regal}, it seems reasonable to believe that their proof could be adapted to obtain a $O(\ln(T))$ bound as is done by \citep[Theorem 4]{Jaksch10}. Although this would contradict our lemma, we noticed a major mistake in the proof of Lemma 11 that may explain the mismatch. We also noticed that \citet{pmlr-v28-maillard13} probably tried to correct this mistake but we identified a similar problem in their proof that we were unable to fix. Since these mistakes are a bit technical, the interested reader may refer to App.~\ref{app:} for further details. We conjecture that regularising by the bias span may not allow to learn non-communicating MDPs. In Sec.~\ref{sec:tucrl} we present a completely different research direction to address this problem.

==> sec_state_art.tex <==
% !TEX root = tucrl.tex

\section{Exploration-exploitation in RL: state-of-the-art}

 As mentioned in introduction, the two main approaches that come with theoretical guarantees in RL are \emph{OFU} in the \emph{frequentist} framework and \emph{PS} in the \emph{Bayesian} framework. In this section, we give a brief overview of state-of-the-art results in both settings.
 
 \textbf{OFU.} Most optimistic learning algorithms in RL are variants of the \ucrl algorithm \citep{Jaksch10}. \ucrl works by episodes and at each episode plays (one of) the (stationary) gain-optimal policy(ies) $\wt{\pi}$ of the MDP $\wt{M}$ with highest optimal gain among all ``plausible'' MDPs. The set of plausible MDPs $\mathcal{M}$ is constructed using confidence intervals (see Sec.~\ref{sec:tucrl}) so as to ensure that with high probability, it contains the true unknown MDP $M^*$. When $M^* \in \mathcal{M}$, it is straightforward to show that $g_{\wt{M}}^* \geq g_{M^*}^*$. \ucrl is thus \emph{gain-optimistic} and its regret can be bounded with probability at least $1-\delta$ by $O(D\sqrt{\Gamma S A T \ln(T/\delta)})$\footnote{The original bound derived by \citet[Theorem 2]{Jaksch10} was $O(DS\sqrt{AT\ln(T/\delta)})$ but \citet{fruit2018constrained} pointed out that a small change in the confidence intervals allows to replace $S$ by $\sqrt{\Gamma S} \leq S$.}. Unfortunately when $M^*$ is non-communicating (\ie when $D =+\infty$), some states will never be visited. $\mathcal{M}$ will then always contain an action that loops on these \emph{fully unknown} states with probability $1$ and reward $\rmaxbound$. As a consequence, \ucrl is way too optimistic ($g_{\wt{M}}^* =\rmaxbound$) and suffers linear regret (both in theory and in practice) \ie \ucrl is unable to \emph{learn}. The first attempt in the literature to overcome this major limitation was proposed by \citet{Bartlett2009regal} who derived three ``pseudo-algorithms''\footnote{None of these ``algorithms'' is actually implementable for various reasons, see \citep{fruit2018constrained} for further details.}: \regal, \regalc and \regald. The idea of \regal was to penalise the optimism on $g^*$ by the optimal bias span $\SP{h^*}$ \ie find the MDP $\wt{M}'\in \mathcal{M}$ that maximises $g_{M}^* - \lambda \cdot \SP{h_{M}^*}$ where $\lambda\geq 0$ is a regularisation coefficient. The term $\SP{h^*}$ can be interpreted as a measure of the \emph{complexity} of the environment: the bigger $\SP{h^*}$, the more difficult it is to achieve the stationary reward $g^*$ by following the optimal policy. In \emph{supervised learning}, regularisation is often used to penalise the objective function by a measure of the complexity of the model so as to avoid \emph{overfitting}. It is thus reasonable to expect that \emph{over-optimism} in online RL can also be avoided through regularisation. The regret bound of \regal holds only when $\lambda$ is set to $\Theta (1/\sqrt{l_k})$ where $l_k$ is the length of the future episode. Unfortunately, an episode stops when the number of visits in a state-action pair $(s,a) \in \calS \times \mathcal{A}$ has doubled and it is not possible to predict the future sequence of states of a given policy for two reasons: 1) the true MDP $M^*$ is unknown and 2) what is observed is a random \emph{sampled} trajectory (as opposed to \emph{expected}). As a result, \regal is not \emph{implementable}. \citet{Bartlett2009regal} proposed an alternative algorithm -- \regald -- that leverages on the \emph{doubling trick} to guess the value of $l_k$ and proved a slightly worse regret bound than for \regal. The idea of \regalc is to incorporate prior knowledge into \ucrl to not only be able to learn when $D = +\infty$, but also improve the regret when $D <+\infty$. More precisely, \regalc takes as input a finite upper-bound $H<+\infty$ on the optimal bias span of the true MDP $\SP{h^*}$\footnote{By definition, $\SP{h^*}<+\infty$ for any MDP (even if $D = +\infty$).}. As a result, the regret guarantees of \regalc are identical to those of \ucrl with $\rmaxbound D$ replaced by $\min\{H,\rmaxbound D\}$. \citet[Theorem 4]{Bartlett2009regal} also showed that $\SP{h^*} \leq \rmaxbound D$ and in many MDPs $\SP{h^*}$ is actually much smaller than $\rmaxbound D$. Therefore, if $H$ is close enough to $\SP{h^*}$, the improvement of \regalc over \ucrl is potentially huge. Unfortunately, \regalc involves solving a complex optimisation problem that is probably intractable. Recently, \citet{fruit2018constrained} relaxed the optimisation problem solved by \regalc and derived an efficient algorithm -- \scal -- that enjoys the same theoretical guarantees as \regalc. 
 
 Although this would contradict our lemma, we noticed a major mistake in the proof of Lemma 11 that may explain the mismatch. We also noticed that \citet{pmlr-v28-maillard13} probably tried to correct this mistake but we identified a similar problem in their proof that we were unable to fix. Since these mistakes are a bit technical, the interested reader may refer to App.~\ref{app:} for further details. We conjecture that regularising by the bias span may not allow to learn non-communicating MDPs. In Sec.~\ref{sec:tucrl} we present a completely different research direction to address this problem.
 
 \textbf{PS.} There is also an extensive literature on Bayesian methods for RL (Posterior sampling) with guarantees on the expected Bayesian regret usually. We briefly discuss state-of-the-art approaches
 
 In conclusion, it is still an opened question whether regret bounds can be derived when no upper-bound on $\SP{h^*}$ is available. We answer positively to this question in this paper....
 
%  It is easy to verify theoretically and empirically that when the MDP is not communicating (\ie when $D = +\infty$), the regret of \ucrl grows linearly with $T$ (\ie ${T}_M^\dagger = {T}_M^* = +\infty$). In this case, \ucrl never \emph{learns} (refer to Sec.~\ref{sec:regal} for a more detailed explanation). The first attempt in the literature to overcome this major limitation was proposed by \citet{Bartlett2009regal} who derived three ``pseudo-algorithms''\footnote{None of these ``algorithms'' is actually implementable for various reasons, see \citep{fruit2018constrained} for further details.}: \regal, \regalc and \regald. We postpone the discussion about \regal and \regald to Sec.~\ref{sec:regal} and restrict attention to \regalc for now. The idea of \regalc is to incorporate prior knowledge into \ucrl to not only be able to learn when $D = +\infty$, but also improve the regret when $D <+\infty$. More precisely, \regalc takes as input a finite upper-bound $H<+\infty$ on the optimal bias span of the true MDP $\SP{h^*}$\footnote{By definition, $\SP{h^*}<+\infty$ for any MDP (even if $D = +\infty$).}. As a result, the regret guarantees of \regalc are identical to those of \ucrl with $\rmaxbound D$ replaced by $\min\{H,\rmaxbound D\}$. \citet[Theorem 4]{Bartlett2009regal} also showed that $\SP{h^*} \leq \rmaxbound D$ and in many MDPs $\SP{h^*}$ is actually much smaller than $\rmaxbound D$. Therefore, if $H$ is close enough to $\SP{h^*}$, the improvement of \regalc over \ucrl is potentially huge. Unfortunately, \regalc involves solving a complex optimisation problem that is probably intractable. Recently, \citet{fruit2018constrained} relaxed the optimisation problem solved by \regalc and derived an efficient algorithm -- \scal -- that enjoys the same theoretical guarantees as \regalc. Although they only provide an analogue of Theorem 2 of \citet{Jaksch10} (Theorem 12) \ie a $O(\sqrt{T})$ regret bound with $D$ replaced by $H$, it seems straightforward to extend their result to a $O(\ln({T}))$ regret bound (analogue of Theorem 4 of \citet{Jaksch10} with $D$ replaced by $H$). It is still an opened question whether the same guarantees can be derived when no upper-bound on $\SP{h^*}$ is available. We will not provide an answer to this question but we will show in the next section that when $D = +\infty$ and $\SP{h^*}$ is unknown, any \emph{efficient} learning algorithm must be such that ${T}_M^* =+\infty$.
% In this paper, we focus on \emph{frequentist} regret guarantees and algorithms using OFU. 
% We conclude Sec.~\ref{sec:limits} with a discussion on regularised optimistic approaches in RL, first introduced by \citet{Bartlett2009regal} for exploration-exploitation in weakly-communicating MDPs and then used in other contexts (see for example \citep{pmlr-v28-maillard13}). \ucrl works by episodes and at each episode plays a (stationary) gain-optimal policy $\wt{\pi}$ of the MDP $\wt{M}$ with highest optimal gain among all ``plausible'' MDPs. The set of plausible MDPs $\mathcal{M}$ is constructed using confidence intervals (see Sec.~\ref{sec:tucrl}) so as to ensure that with high probability, it contains the true unknown MDP $M^*$. When $M^* \in \mathcal{M}$, it is straightforward to show that $g_{\wt{M}}^* \geq g_{M^*}^*$ and so \ucrl is \emph{gain-optimistic}. Unfortunately when $M^*$ is non-communicating, some states will never be visited. $\mathcal{M}$ will then always contain an action that loops on these states with probability $1$ and reward $\rmaxbound$. As a consequence, \ucrl is way too optimistic ($g_{\wt{M}}^* =\rmaxbound$) and suffers linear regret. To avoid this problem, the intuition of \citet{Bartlett2009regal} was to penalise the optimism on $g^*$ by the optimal bias span $\SP{h^*}$ \ie find the MDP $\wt{M}'\in \mathcal{M}$ that maximises $g_{M}^* - \lambda \cdot \SP{h_{M}^*}$ where $\lambda\geq 0$ is a regularisation coefficient. The term $\SP{h^*}$ can be interpreted as a measure of the \emph{complexity} of the environment: the bigger $\SP{h^*}$, the more difficult it is to achieve the stationary reward $g^*$ by following the optimal policy. In \emph{supervised learning}, regularisation is often used to penalise the objective function by a measure of the complexity of the model so as to avoid \emph{overfitting}. It is thus reasonable to expect that \emph{over-optimism} in online RL can also be avoided through regularisation. The regret bound of \regal holds only when $\lambda$ is set to $\Theta (1/\sqrt{l_k})$ where $l_k$ is the length of the future episode. Unfortunately, an episode stops when the number of visits in a state-action pair $(s,a) \in \calS \times \mathcal{A}$ has doubled and it is not possible to predict the future sequence of states of a given policy for two reasons: 1) the true MDP $M^*$ is unknown and 2) what is observed is a random \emph{sampled} trajectory (as opposed to \emph{expected}). As a result, \regal is not \emph{implementable}. \citet{Bartlett2009regal} proposed an alternative algorithm -- \regald -- that leverages on the \emph{doubling trick} to guess the value of $l_k$ and proved a slightly worse regret bound than for \regal. 
% Nevertheless, in Ex.~\ref{ex:weakly_communicating}, knowing the length of an episode (at least on expectation) seems to be equivalent to knowing $\varepsilon$ (or at least knowing whether $\varepsilon =0$ or $\varepsilon >0$ which is the main issue as discussed in Sec.~\ref{sec:no_free_lunch}). According to Lem.~\ref{lem:weakly_communicating}, this would imply that \regald does not admit any $O(\ln(T)^\beta)$ regret bound (for arbitrary $\beta>0$). Although such a bound is never proved by \citet{Bartlett2009regal}, it seems reasonable to believe that their proof could be adapted to obtain a $O(\ln(T))$ bound as is done by \citep[Theorem 4]{Jaksch10}. Although this would contradict our lemma, we noticed a major mistake in the proof of Lemma 11 that may explain the mismatch. We also noticed that \citet{pmlr-v28-maillard13} probably tried to correct this mistake but we identified a similar problem in their proof that we were unable to fix. Since these mistakes are a bit technical, the interested reader may refer to App.~\ref{app:} for further details. We conjecture that regularising by the bias span may not allow to learn non-communicating MDPs. In Sec.~\ref{sec:tucrl} we present a completely different research direction to address this problem.

==> sec_state_art2.tex <==
% !TEX root = tucrl.tex

\section{Exploration-exploitation in RL: state-of-the-art}\label{sec:state_art}
 
 As mentioned in introduction, the two main approaches that come with theoretical guarantees in RL are \emph{OFU} in the \emph{frequentist} framework and \emph{PS} in the \emph{Bayesian} framework. In this section, we give a brief overview of state-of-the-art results in both settings.
 
 \textbf{OFU.} Most optimistic learning algorithms in RL are variants of the \ucrl algorithm \citep{Jaksch10}. \ucrl works by episodes and at each episode plays (one of) the (stationary) gain-optimal policy $\wt{\pi}$ of the MDP $\wt{M}$ with highest optimal gain among all ``plausible'' MDPs.
 The set of plausible MDPs $\mathcal{M}$ is constructed using confidence intervals (see Sec.~\ref{sec:tucrl}) so as to ensure that with high probability, it contains the true unknown MDP $M^*$. When $M^* \in \mathcal{M}$, it is straightforward to show that $g_{\wt{M}}^* \geq g_{M^*}^*$.
 \ucrl is thus \emph{gain-optimistic} and its regret can be bounded with probability at least $1-\delta$ by $O(D\sqrt{\Gamma S A T \ln(T/\delta)})$\footnote{The original bound derived by \citet[Theorem 2]{Jaksch10} was $O(DS\sqrt{AT\ln(T/\delta)})$ but \citet{fruit2018constrained} pointed out that a small change in the confidence intervals allows to replace $S$ by $\sqrt{\Gamma S} \leq S$.}. 
 Unfortunately when $M^*$ is non-communicating (\ie when $D =+\infty$), some states will never be visited. $\mathcal{M}$ will then always contain an action that loops on these \emph{fully unknown} states with probability $1$ and reward $\rmaxbound$. As a consequence, \ucrl is way too optimistic ($g_{\wt{M}}^* =\rmaxbound$) and suffers linear regret (both in theory and in practice) \ie \ucrl is unable to \emph{learn}. The first attempt in the literature to overcome this major limitation was proposed by \citet{Bartlett2009regal} who derived three ``pseudo-algorithms''\footnote{None of these ``algorithms'' is actually implementable for various reasons, see \citep{fruit2018constrained} for further details.}: \regal, \regalc and \regald. 
 The idea of \regal was to penalise the optimism on $g^*$ by the optimal bias span $\SP{h^*}$ \ie find the MDP $\wt{M}'\in \mathcal{M}$ that maximises $g_{M}^* - \lambda \cdot \SP{h_{M}^*}$ where $\lambda\geq 0$ is a regularisation coefficient. 
 In \emph{supervised learning}, regularisation is often used to penalise the objective function by a measure of the complexity of the model so as to avoid \emph{overfitting}. Here the goal is to avoid \emph{over-optimism}. The term $\SP{h^*}$ can be interpreted as a measure of the \emph{complexity} of the environment: the bigger $\SP{h^*}$, the more difficult it is to achieve the stationary reward $g^*$ by following the optimal policy. 
 \regal achieves a high probability regret bound of $O(\SP{h^*}S\sqrt{AT\ln(T/\delta)})$ \citep[Theorem 1]{Bartlett2009regal} when $\lambda$ is set to $\Theta (1/\sqrt{\ell_k})$ where $\ell_k$ is the length of the future episode. 
 Unfortunately, an episode stops when the number of visits in a state-action pair $(s,a) \in \calS \times \mathcal{A}$ has doubled and it is not possible to predict the future sequence of states of a given policy for two reasons: 1) the true MDP $M^*$ is unknown and 2) what is observed is a random \emph{sampled} trajectory (as opposed to \emph{expected}). As a result, \regal is not \emph{implementable}.
 To solve this problem, \citet{Bartlett2009regal} proposed an alternative algorithm -- \regald -- that leverages on the \emph{doubling trick} to guess the value of $\ell_k$ and proved a slightly worse regret bound than for \regal: $O\Big(\SP{h^*}\sqrt{S^3 AT\ln^2(T/\delta)}\Big)$ \citep[Theorem 3]{Bartlett2009regal}. However, we noticed a major mistake in the proof of  \citep[Theorem 3]{Bartlett2009regal} that we believe questions the validity of this regret bound.
 We also noticed that \citet{pmlr-v28-maillard13} probably tried to correct this mistake but we identified a similar problem in their proof that we were unable to fix. The interested reader may refer to App.~\ref{app:mistake_regal} for further details on these mistakes. 
 \emph{We therefore conjecture that regularising by the bias span may not allow to learn non-communicating MDPs} ($D = +\infty$). The last idea suggested by \citet{Bartlett2009regal} was to incorporate prior knowledge into \ucrl. \regalc takes as input a finite upper-bound $H<+\infty$ on the optimal bias span $\SP{h^*}$ of the true MDP \footnote{By definition, $\SP{h^*}<+\infty$ for any MDP (even if $D = +\infty$).} and achieves the same regret guarantees as \ucrl with $\rmaxbound D$ replaced by $\min\{H,\rmaxbound D\}$. \citet[Theorem 4]{Bartlett2009regal} also showed that $\SP{h^*} \leq \rmaxbound D$ and in many MDPs $\SP{h^*}$ is actually much smaller than $\rmaxbound D$ implying that the improvement of \regalc over \ucrl is potentially huge.
 Unfortunately, \regalc involves solving a complex optimisation problem that is probably intractable. Recently, \citet{fruit2018constrained} relaxed the optimisation problem solved by \regalc and derived an efficient algorithm -- \scal -- that enjoys the same theoretical guarantees as \regalc. Not only \scal can \emph{learn} when $D = +\infty$, but it always performs at least as well as \ucrl when $D <+\infty$.
 
 \textbf{PS.} \citet{Strens00abayesian} studies PS in the infinite horizon discounted setting while \citet{Osband2013more} consider finite horizon. We restrict attention to the infinite horizon undiscounted setting (gain optimality) where, unlike \citet{DBLP:conf/colt/GopalanM15}, we do not assume the existence of a recurrent state under any stationary policy. To the best of our knowledge, the only regret guarantees available in the literature for this setting are \citep{Abbasi-Yadkori:2015:BOC:3020847.3020849} and \citep{NIPS2017_6732}. However, the counter-example of \citet{DBLP:journals/corr/OsbandR16a} invalidates the result of \citet{Abbasi-Yadkori:2015:BOC:3020847.3020849}. \citet{NIPS2017_6732} present a PS algorithm with expected \emph{Bayesian} regret bounded as $O(HS\sqrt{AT\ln(T)})$. The constant $H$ appearing in the regret bound is an upper-bound on the optimal bias span of all the MDPs for which the density function of the prior distribution is non-zero. In \citep[Remark 1]{NIPS2017_6732}, the authors claim that their algorithm do not require the knowledge of $H$ to derive the regret bound. However, in App.~\ref{app:unbounded.span.bayesian} we show on a very simple example that for most continuous prior distributions (\eg uninformative priors like Dirichlet), it is very likely that $H =+ \infty$ implying that the regret bound does not hold. As a consequence, the prior distribution should contain a lot of information about $\SP{h^*}$ for the bound to hold. Finally, \citet{Agrawal2017posterior} introduced an \emph{optimistic} version of PS which achieves the same regret guarantees as \ucrl (on the frequentist regret) for communicating MDPs only.
 
 \todor{Check whether there is no other result for PS. It's a bit depressing so far...}
 \todom{There is also Yasin recent paper~\citep{theocharous2017largeps}}
 
 In conclusion, we conjecture that with current state-of-the-art techniques of proof, no existing algorithm can be proved to achieve sub-linear regret in a general weakly communicating MDP (either in the Bayesian or frequentist setting) without some form of prior knowledge (\eg $D < +\infty$, known upper-bound $H\geq \SP{h^*}$, etc). In Sec.~\ref{sec:tucrl} we will present what we believe is a completely novel approach to address the problem of learning weakly-communicating MDPs \emph{without prior knowledge}.
 
 


==> sec_tucrl.tex <==
% !TEX root = tucrl.tex

\section{Truncated Upper-Confidence for Reinforcement Learning (NEW)}
In this section we introduce \tucrl, an optimistic online RL algorithms that is able to efficiently balance exploration and exploitation in order to learn in weakly communicating MDPs without prior knowledge. 
Since our proposed algorithm \tucrl is a variant of \ucrl, we first recall their common structure summarized in Fig.~\ref{fig:ucrl.constrained}.
%
\begin{figure}[t]
\renewcommand\figurename{\small Figure}
\begin{minipage}{\columnwidth}
\bookboxx{
\textbf{Input:} Confidence $\delta \in ]0,1[$, $r_{\max}$, $\calS$, $\A$, a constant $c \geq 0$

\noindent \textbf{Initialization:} Set $N_1(s,a) = 0$ for any $(s,a) \in \calS \times \A$, $t = 1$ and observe $s_1$.

\noindent \textbf{For} episodes $k=1, 2, ...$ \textbf{do}

\begin{enumerate}[leftmargin=4mm,itemsep=0mm]
\item Set $t_k = t$ and episode counters $\nu_k (s,a) = 0$

\item Compute estimates $\wh{p}_k(s' | s,a)$, $\wh{r}_k(s,a)$ and a confidence set~$\mathcal{M}_k$ (\ucrl, \regalc), resp.~$\mathcal{M}_k^\diamond$ (\tucrl)
%$\wt{\mathcal{M}}_k^\ddagger$ (based on Thm.~\ref{def:augmented.perturbed.mdp} with $\eta = 1/\sqrt{t_k}$)

\item
% Compute (an approximation of) the optimal policy $\widetilde{\pi}_k$ and the optimistic MDP $\widetilde{M}_k$, that is,
% $$(\wt{M}^*_k, \wt\pi^*_k ) \in \argmax_{M\in\mathcal{M}_k, \pi} g^\pi_M.$$
Compute an $\rmaxbound/\sqrt{t_k}$-approximation $\widetilde{\pi}_k$ of the solution of Eq.~\ref{eq:ucrl.optimization} (\ucrl), resp. Eq.~\ref{eq:optimistic.policy.regalc} (\regalc), resp. Eq.~\ref{eq:tucrl.optimization} (\tucrl)

%\item Use \regopt to compute an $1/\sqrt{t_k}$-approximation $\widetilde{\pi}_k$ of the solution of Eq.~\ref{eq:optimistic.policy.relaxedregalc} where $\mathcal{M}_k$ is replaced by $\mathcal{M}_k^{\ddagger}$ 
%
\item Sample action $a_t \sim \pi_k(\cdot|s_t)$

\item \textbf{While} 
%        $\nu_k(s_t,a_t) \leq \max\{1, N_k(s_t,a_t)\}$ 
        \textit{ stopping\_condition }
        \textbf{do}
%
\begin{enumerate}[leftmargin=4mm,itemsep=-1mm]
        \item Execute $a_t$, obtain reward $r_{t}$, and observe $s_{t+1}$
        \item Set $\nu_k (s_t,a_t) \pluseq 1$ 
        \item Sample action $a_{t+1} \sim \wt{\pi}_k(\cdot|s_{t+1})$ and set $t \pluseq 1$
\end{enumerate}

\item Set $N_{k+1}(s,a) = N_{k}(s,a)+ \nu_k(s,a)$ \tikz[baseline]{\node[anchor=base](alg_lastline){};}
\end{enumerate}
}
\caption{\small The general structure of optimistic algorithms for RL.}
\label{fig:ucrl.constrained}
\begin{tikzpicture}[overlay,font=\small]
        \draw[anchor=south west, draw=black] ($(alg_lastline) + (2cm,-0.2cm)$) rectangle ($(alg_lastline) + (8cm, 2.5cm)$);
        \coordinate (A) at ($(alg_lastline) + (2.3cm, 2.1cm)$);
        \node[anchor=west] at (A) {$\triangleright$~\emph{stopping\_condition} (\ucrl, \regalc)};
        \node[anchor=west] at ($(A)+(0.3cm,-.5cm)$) {$\nu_k(s_t,a_t) \leq \max\{1, N_k(s_t,a_t)$};
        % TUCRL
        \node[anchor=west] (TUCRL_stop) at ($(A)+(0, -1.cm)$) {$\triangleright$~\emph{stopping\_condition} (\tucrl)};
        \node[anchor=west] at ($(A)+(0.3cm,-1.4cm)$) {$t_k == t$ \textbf{or} $\Big( \sum_{a \in \A_{s_t}} N_k(s_t,a) > 0$ };
        \node[anchor=west] at ($(A)+(0.3cm,-2.cm)$) { \textbf{ and }$\nu_k(s_t,a_t) \leq \max\{1, N_k(s_t,a_t)\} \Big)$};
\end{tikzpicture}
\end{minipage}
\end{figure}

\tucrl proceeds through episodes $k=1,2\dots$ At the beginning of each episode $k$, \tucrl constructs the empirical estimates of $\calScom$ and $\calStrans$ \ie the set of communicating and transient states in $M^*$:
\begin{align*}
        \calScom_k := \left\{s \in \calS \;\big|\; \sum_{a \in \A_s} N_k(s,a) > 0 \right\} \cup \{s_{t_k}\}, \qquad\quad
        \calStrans_k := \calS \setminus \calScom_k,
\end{align*}
where $t_k$ is the starting time of episode $k$.
Then, \tucrl builds a set of \emph{constrained} MDPs $\mathcal{M}_k^2 = \big\{ M = \langle \calS, \A, \wt{r}, \wt{p}\rangle \;:\; \forall (s,a)\in \calS \times \A,~\wt{r}(s,a) \in B_{r,k}(s,a), \wt{p}(s'|s,a) \in B_{p,k}^2(s,a,s'),~ \wt{p}(\cdot|s,a) \in \mathcal{C} \big\}$  where $\mathcal{C} = \{p \in \mathbb{R}^S | \forall s,~p(s) \geq 0 \wedge \sum_{s} p(s) = 1\}$ is the $(S-1)$-simplex.
Let $B_{r,k}$ and $B_{p,k}^1$ be high-probability confidence intervals on the rewards and transition probabilities of the true MDP $M^*$, then:
\begin{equation*}
        B_{p,k}^2(s,a,s') = \begin{cases}
                \{0\} & \text{if } (s,a,s') \in \left( (\calS \times \A) \setminus \mathcal{K} \right) \times \calStrans_k\\
                B_{p,k}^1(s,a,s') & \text{otherwise} % \forall (s,a,s') \in \{\calS \times \A \times \calScom_k\} \cup \{(\mathcal{K} \cup (\calStrans_k \times \A)) \times \calStrans_k \}
        \end{cases}
\end{equation*}
where $\mathcal{K} = \Big\{ (s,a) \in \calScom_k \times \A \,:\, N_k^\pm(s,a) \leq \sqrt{\sfrac{t_k}{SA}} \Big\}$ contains the state-action pairs that are currently non-sufficiently explored.
For these pairs, it is \emph{plausible} it may exist a transition to a state $s'$ that has never been observed (\ie $s' \in \calStrans_k$).
We denote by $\mathcal{M}_k^1$ the set of plausible MDPs constructed by \ucrl using $B_{r,k}$ and $B_{p,k}^1$, which guarantees that $M^* \in \mathcal{M}_k^1$ w.h.p.
In this paper we use confidence intervals constructed using the empirical Bernstein's inequality~\citep{audibert2007tuning,Maurer2009empirical}
\begin{align*}
\beta_{r,k}^{sa}
:=
         \sqrt{\frac{14 
                         \wh{\sigma}_{r,k}^2(s,a)
%        \ln(2 SA t_k/\delta)
                        b_{k,\delta}
                }{
%        \max\lbrace 1, N_k(s,a)\rbrace
        N^{+}_k(s,a)
}} + \frac{\frac{49}{3}
%                 \alpha_r 
\rmaxbound
%        \ln(2 SA t_k/\delta)
        b_{k,\delta}
        }{
        N^{\pm}_k(s,a)
%        \max\lbrace 1, N_k(s,a)-1 \rbrace
}
, \qquad
\beta_{p,k}^{sas'}
:= 
\sqrt{\frac{14 \wh{\sigma}_{p,k}^2(s'|s,a) 
%        \ln(2 SA t_k/\delta)
                        b_{k,\delta}
                }{
%        \max\lbrace 1, N_k(s,a)\rbrace
        N^{+}_k(s,a)
}
} +\frac{\frac{49}{3}
%                 \alpha_p 
%        \ln(2 SA t_k/\delta)
        b_{k,\delta}
        }{
        N^{\pm}_k(s,a)
%        \max\lbrace 1,N_k(s,a)-1 \rbrace
}
\end{align*}
where $N_k(s,a)$ is the number of visits in $(s, a)$ before episode $k$, 
$N^{+}_k(s,a) := \max\lbrace 1, N_k(s,a) \rbrace$, 
$N^{\pm}_k(s,a) := \max\lbrace 1, N_k(s,a)-1 \rbrace$, 
$\wh{\sigma}_{r,k}^2(s,a)$ and $\wh{\sigma}_{p,k}^2(s'|s,a)$ are the empirical variances of $r(s,a)$ and ${p}(s'|s,a)$ %respectively 
% (formally defined in eqn.~\eqref{eqn:def_empirical_variance} of App.~\ref{app:regret.reg.ucrl}) 
and $b_{k,\delta} = \ln(2 SA t_k/\delta)$.
%
Given the empirical averages $\wh{r}_k(s,a)$ and $\wh{p}_k(s'|s,a)$ of rewards and transitions, we define $B_{r,k}(s,a) := [\wh{r}_k(s,a) - \beta_{r,k}^{sa}, \wh{r}_k(s,a) + \beta_{r,k}^{sa}] \cap [0, \rmaxbound]$ and $B_{p,k}^1(s,a,s') := [\wh{p}_k(s'|s,a) - \beta_{p,k}^{sas'},\wh{p}_k(s'|s,a) + \beta_{p,k}^{sas'}] \cap [0,1]$.

Finally, we introduce \emph{relaxations} of the extended MDPs that consider the $\ell_1$-norm concentration inequality around $p(\cdot|s,a)$ instead of $S$ concentration inequalities around $p(s'|s,a)$ for all $s'\in \calS$.
We will denote by $\mathcal{M}^{1+}_k$ and  $\mathcal{M}_k^{2+}$ the relaxation of $\mathcal{M}_k^1$ and $\mathcal{M}_k^2$, respectively.
Then, for $i \in \{1,2\}$, 
$\mathcal{M}_k^{i+} = \Big\{ M = (\calS,\A, \wt{r}, \wt{p}) :\;
        \wt{r}(s,a) \in B_{r,k}^{i+}(s,a), \;
                        \wt{p}(\cdot|s,a) \in B_{p,k}^{i+}(s,a) \Big\}$
where the reward intervals are not altered (\ie $B_{r,k}^{i+} = B_{r,k}^{i}$) and, for any $(s,a) \in \calS \times \A$
\begin{align*}
        B_{p,k}^{1+}(s,a) 
        &= \left\{ 
                \wt{p}(\cdot|s,a)\in \mathcal{C} :~
%                \wt{p}\in \mathbb{R}^S :~ \wt{p}(\cdot|s,a)\in \mathcal{C} \wedge
                \| \wt{p}(\cdot|s,a) - \wh{p}(\cdot|s,a) \|_1 \leq \beta_{p,k}^{sa} := \sum_{s'\in\calS}\beta_{p,k}^{sas'}
        \right\},\\
        B_{p,k}^{2+}(s,a) 
        &= \begin{cases}
        B_{p,k}^{1+}(s,a) \cap \left\{\wt{p} \in \mathcal{C} :~ \sum_{s' \in \calStrans_k} \wt{p}(s'|s,a) = 0  \right\} & \text{if }(s,a) \in \mathcal{K}\\
                B_{p,k}^{1+}(s,a) & \text{otherwise} %(s,a) \in (\calS \times \A) \setminus \mathcal{K}\\
        \end{cases}
\end{align*}

Then, \tucrl considers a variation of the \ucrl problem defined as:
\begin{equation}
        \label{eq:tucrl.optimization}
        (\wt{M}_k, \wt{\pi}_k) = \argmax_{M \in \mathcal{M}_k^\diamond, \pi \in \Pi^{\textsc{SD}}(M)} \{g^{\pi}_M\} 
        \qquad \text{where } \quad \mathcal{M}_k^\diamond = \begin{cases}
                \mathcal{M}_k^{2} & \text{if } \calStrans_k = \emptyset\\
                \mathcal{M}_k^{2+} & \text{otherwise}
        \end{cases}
\end{equation}
%
Similarly to \ucrl, problem~\eqref{eq:tucrl.optimization} is equivalent to finding $\wt{\mu}^* \in \argmax_{\mu \in \SD(\wt{\mathcal{M}}_k)} \big\lbrace g^\mu_{\wt{\mathcal{M}}_k} \big\rbrace$ where $\wt{\mathcal{M}}_k$ is the \emph{extended} MDP (sometimes called \emph{bounded-parameter} MDP) implicitly defined by $\mathcal{M}_k^{\diamond}$.
This problem can be solved up to an $\epsilon_k$-approximation ($\epsilon_k = \rmaxbound/\sqrt{t_k}$) using extended value iteration (EVI) on $\mathcal{M}_k^{\diamond}$.
Starting from an initial vector $u_0 = 0$, EVI iteratively applies the optimal Bellman operator of $\mathcal{M}_k^{\diamond}$: $u_{n+1} = \wt{L}_{\mathcal{M}_k^{\diamond}} u_n$.
Note that when $\calStrans_k = \emptyset$, $\wt{L}_{\mathcal{M}_k^{\diamond}} = \wt{L}_{\mathcal{M}_K^1}$ (see~\citep[][Eq. 5]{Jaksch10}). Otherwise, $\wt{L}_{\mathcal{M}_k^{\diamond}} = \wt{L}_{\mathcal{M}_K^{2+}}$ where, for any $v \in \mathbb{R}^S$:
\begin{equation}\label{eq:Lop_m2plus}
\begin{aligned}
        \wt{L}_{\mathcal{M}_k^{2+}}v(s) &:= \max_{a \in \A_s} \left\{
                \max_{\wt{r} \in B_{r,k}(s,a)} \wt{r} +  (\wt{p}^{sa})^\transp v
        \right\}
\end{aligned}
\end{equation}
and $\wt{p}^{sa} = \argmax_{\wt{p} \in B_{p,k}^{2+}(s,a)} \{\wt{p}^T v_{n}\}$ can be solved using~\citep[][Fig. 2]{Jaksch10} except when $(s,a) \in \mathcal{K}$ in which case we restrict the algorithm to work on $\calScom_k$ since $\wt{p}^{sa}(s') := 0$ for any $s' \in \calStrans_k$ (see App.~\ref{} and Alg.~\ref{alg:opt.prob.h} for details).
If EVI is stopped when $sp_{\calScom_k}\left\{u_{n+1} - u_n\right\} \leq \epsilon_k$ and the true MDP is sufficiently explored, then the greedy policy $\wt{\mu}_k$ \wrt $u_n$ is $\epsilon_k$-optimal, \ie $g^{\wt{\mu}_k}_{\wt{\mathcal{M}}_k} \geq g^*_{\wt{\mathcal{M}}_k} \geq g^*_{M^*} - \epsilon_k$ (see Sec.~\ref{sec:sketch.regret.proof} for details).
Finally, note that when the true MDP $M^*$ is communicating, there exists an episode $\wb{k}$ \st for all $k \geq \wb{k},~\calStrans_k = \emptyset$ and
\tucrl will behave like \ucrl with the tightest possible confidence intervals (\ie $ \mathcal{M}_k^\diamond =  \mathcal{M}_k^2 =  \mathcal{M}_k^1$).

We are now ready to prove the following regret bound (see App.~\ref{app:tucrl.regret}).

\begin{theorem}\label{thm:tucrl.regret}
        For any weakly communicating MDP $M$, with probability at least $1-\delta$ it holds that for any $T > 1$, the regret of \tucrl is bounded as
        \[
                \Delta(\tucrl,T) = \mathcal{O} \left(\rmaxbound D_c \sqrt{\nextstates SA T \ln\left( \frac{SAT}{\delta} \right)} + \rmaxbound D_c^2 S^3 A \ln^2\left( \frac{SAT}{\delta} \right) \right).
        \]
%        where $C$ is a numerical constant independent of the MDP $M$.
\end{theorem}
\todom{Comments on the regret}

\subsection{Analysis of \tucrl} \label{sec:sketch.regret.proof}
This section aims to provide a rough outline of the main steps required to prove Thm.~\ref{thm:tucrl.regret}.
The analysis of \tucrl is detailed in App.~\ref{app:tucrl.regret} and leverages on the structure used for \ucrl~\citep{Jaksch10}.
The main difference is due to the use of the \emph{truncated} extended MDP $\mathcal{M}_k^{2+}$ which implies that the statistical argument may fail (\ie if $\calStrans_k \neq \emptyset$, the true MDP $M^*$ might not be included in $\mathcal{M}_k^{2+}$). We will show how to treat this case based on the exploration level of an episode $k$.

In particular, 
%\textbf{Linear phase:} 
\tucrl suffers \textbf{linear regret} in all the episodes with a non-sufficient level of exploration (\ie episodes $k$ s.t. $t_k < C(k) = \mathcal{O}\left(D_c^2 S^3A\ln^2(\sfrac{2SAt_k}{\delta})\right)$).
Since the overall number of times this event happens is ``small'', the contribute to the cumulative regret is polylogarithmic: $\sum_{k=1}^m \Delta_k \cdot \mathbbm{1}\lbrace t_k < C(k) \rbrace = \mathcal{O}(\rmaxbound D_c^2S^3A\ln^2\left(\sfrac{2SAT}{\delta}\right))$ where $\Delta_k$ is the regret in episode $k$.
%
Note that 
% \textbf{Number of episodes:}
% Similarly to \ucrl, the cumulative regret $\Delta(\tucrl,T)$ can be bounded w.h.p.\@\xspace by $\sum_{k=1}^m \Delta_k + \rmaxbound\sqrt{\frac{5}{2}T \ln\left(\frac{8T}{\delta}\right)}$ where $\Delta_k = \sum_{s,a} \nu_k(s,a)\left(g^* - r(s,a)\right)$ is the regret in episode $k$ and $\nu_k(s,a)$ is the number of visits in $(s,a)$ during episode $k$.
the stopping condition used by \tucrl is the original \ucrl one combined with the condition $s_{t} \in \calS_{k_t}^2$ ($k_t$ being the episode associated to time $t$). Then, it is easy to prove (see App.~\ref{app:regret.number.episodes}) that the \textbf{total number of episodes} $m$ is incremented at most by $S$.

% \textbf{Optimism:} 
% we start noticing that when $\calStrans_k = \emptyset$, the true MDP $M^* \in \mathcal{M}_k^1 = \mathcal{M}_k^2 = \mathcal{M}_k^\diamond$ w.h.p. and we can use the same arguments in~\citep{Jaksch10}. When $\calStrans_k \neq \emptyset$, $M^*$ might not be included in $\mathcal{M}_k^\diamond = \mathcal{M}_k^{2+}$.
% To analyse this scenario, we start considering episodes with a non-sufficient level of exploration (\ie $t_k < C(k) = \wt{\mathcal{O}}(D_c^2 S^3A)$), for which \tucrl suffers linear regret.
% Since the overall number of times this event happens is small, the contribute to the cumulative regret is polylogarithmic: $\sum_{k=1}^m \Delta_k \cdot \mathbbm{1}\lbrace t_k < C(k) \rbrace = \mathcal{O}(\rmaxbound D_c^2S^3A\ln^2\left(2SAT/\delta\right))$.
In the case $t_k \geq C(k)$, 
%we can identifies the possible scenarios (see App.~\ref{app:regret.Minset}).
we are able to prove that the solution found by EVI is \textbf{optimistic} for any $\mathcal{M}_k^\diamond$. The following lemma helps to identified the possible cases (see App.~\ref{app:regret.Minset}).
\begin{lemma}
        Let episode $k$ be such that $M^* \in \mathcal{M}^1_k$, $\calStrans_k\neq \emptyset$ and $t_k \geq C(k)$. 
        Then, either $\calStrans_k = \calStrans$ (case I) or there exists a state-action pair $(s,a) \in \calScom_k \times \A$ for which transitions to $\calStrans_k$ are allowed, \ie $N_k^{\pm}(s,a) \leq \sqrt{\sfrac{t_k}{SA}}$ (case II).
\end{lemma}
%As a consequence, either $\calStrans_k = \calStrans$ or there exists a state-action pair $(s,a) \in \calScom_k \times \A$ for which transitions to $\calStrans_k$ are allowed (\ie $N_k^{\pm}(s,a) \leq \sqrt{t_k/(SA)}$). For these two cases, it is possible to prove that the solution to problem~\ref{eq:tucrl.optimization} returned by EVI is \emph{optimistic}.
We start noticing that when $\calStrans_k = \emptyset$, the true MDP $M^* \in \mathcal{M}_k^1 = \mathcal{M}_k^2 = \mathcal{M}_k^\diamond$ w.h.p.
Similarly, if $\calStrans_k = \calStrans$ then $M^* \in \mathcal{M}_k^{2+} = \mathcal{M}_k^\diamond$ w.h.p., since \tucrl only truncates transitions that are already not available in $M^*$.
In both cases,  we can use the same arguments in~\citep{Jaksch10} to prove optimism.
Finally, note that in \emph{case II} the gain of any state $s' \in \calStrans_k$ is $\rmaxbound$ and, since there exists a path from $\calScom_k$ to $\calStrans_k$, the gain of the solution returned by EVI is $\rmaxbound$ (\ie optimistic).

%We report a sketch of the proof. \emph{I)} if $\calStrans_k = \calStrans$ then $M^* \in \mathcal{M}_k^{2+}$ and optimism can be proved as in~\citep[][Sec. 4.3 \& Thm. 7]{Jaksch10}.
%Note that $\mathcal{M}_k^{2+}$ is such that transitions to any $s' \in \calStrans_k$ are forbidden from any state-action pair $(s,a) \in (\calScom_k=\calScom) \times \A$ and this is true (by definition) in $M^*$ (\ie $p(s'|s,a) = \wt{p}(s'|s,a) = 0$). 
%For $(s,a,s') \notin \calScom_k \times \A \times \calStrans_k$, $p(s'|s,a) \in B_{p,k}^{1}(s,a,s') = B_{p,k}^{2}(s,a,s')$, then $p(\cdot|s,a) \in B_{p,k}^{2+}(s,a)$. 
%\emph{II)} noticing that $B_{r,k}^{2+}$ and $B_{p,k}^{2+}$ are such that there exists an MDP $M' \in \mathcal{M}_k^{2+}$ such that any $s' \in \calStrans_k$ is an absorbing state with reward $\rmaxbound$ and all the states $s \in \calScom_k$ are transient states (recall there is a path from $\calScom_k$ to $\calStrans_k$). It is possible to create such an MDP $M'$ since in $\calStrans_k$ the uncertainty is maximal (see App.~\ref{app:regret.Minset} for details). Thus, the gain of $M'$ is $\rmaxbound$. 
%As a consequence, in both cases $\wt{g}_k \geq g^*_{M^*} - \frac{\rmaxbound}{\sqrt{t_k}}$ and by denoting $\wt{\Delta}_k := \sum_{s,a} \nu_k(s,a) (\wt{g}_k - \wt{r}_k(s,a))$, we can further decompose the regret in episode $k$ as:
%\[
%\Delta_k \leq \wt{\Delta}_k + 2\sum_{s,a}\nu_k(s,a) \beta_{r,k}^{sa} + \rmaxbound \sum_{s,a}\frac{\nu_k(s,a)}{\sqrt{t_k}}
%\]

Similarly to \ucrl, by exploiting the optimism and the optimality equation, we further decompose the regret at episode $k$.
We start focusing on the state-action pairs such that $\mathbbm{1}\{N_k^{\pm}(s,a) > \sqrt{\sfrac{t_k}{SA}}\} := \mathbbm{1}_k(s,a)$.
Lem.~\ref{lem:sum.bad.states} will show that the contribute to the cumulative regret is ``small'' in the case the reverse inequality holds.
In this case $\mathbbm{1}_k(s,a)$, the critical step is \textbf{bounding} the term involving \textbf{the optimistic vector} $\wt{h}_k$ computed by EVI (see Sec 4.3.2 in~\citep{Jaksch10} and App. F.6 in~\citep{fruit2018constrained}):
\begin{align*}
        \nu_k(\wt{P}_k -I)\wt{h}_k &= \sum_{s\in \wb{\calS}_k} \nu_k(s,\wt{\pi}_k(s)) \left(\sum_{s'\in \wb{\calS}_k}\wt{p}_k(s'|s,\wt{\pi}_k(s))w_k(s') - w_k(s) \right)
\end{align*}
where $w_k$ is a linear transformation of $\wt{h}_k$. 
Using Holder inequality the sum can be decomposed into the $\ell_1$-norm of the transition probabilities (that can be bounded using a concentration argument) and $sp_{\wb{\calS}_k}\{w_k\}$.
% The latter is the critical term since the $\ell_1$-norm can be bounded using concentration arguments.
% While the former can be bounded using a concentration argument, the span needs to be carefully handled.
In \ucrl, $\wb{\calS}_k = \calS$ and $\SP{w_k} \leq D$~\citep[][Sec. 4.3]{Jaksch10}.
Unfortunately, this results is uninformative when $M^*$ is weakly communicating.
However, using the new stopping condition, the truncation performed by $\mathcal{M}_k^{2+}$ and the condition $\mathbbm{1}_k(s,a)$, we can show that  $\wb{\calS}_k = \calScom_k$ in \tucrl 
and, since $w_k := \wt{h}_k - \min_{s\in\calScom_k}\{\wt{h}_k\}$, 
$sp_{\calScom_k}\{w_k\} = \max_{s\in\calScom_k}\{w_k\}$ is bounded by the diameter of the communicating part of $M^*$ (see App.~\ref{app:regret.Minset}).
We first introduce the following useful lemma (see App.~\ref{app:shortestpath} for details).
\begin{lemma}\label{L:sp.bias_difference}
            For any pair $(s,\wb{s}) \in \calS \times \calScom_k$,
            $\tau_{\mathcal{M}_k^{1+}}(s \to \wb{s}) = \tau_{\mathcal{M}_k^{2+}}(s \to \wb{s})$.
            Moreover, EVI on $\mathcal{M}_k^{2+}$ is such that (starting from the vector $\boldsymbol{0}$): $\wt{h}_k(s') - \wt{h}_k(s) \leq \rmaxbound \cdot \tau_{\mathcal{M}_k^{2+}}(s \to s')$, $\forall s,s' \in \calS$.
\end{lemma}
Since $M^* \in \mathcal{M}_k^{1+}$,  for all $s, s' \in \calScom_k$, $\tau_{\mathcal{M}_k^{1+}}(s \to s') \leq D_c$. Then, as a consequence of Lem.~\ref{L:sp.bias_difference}, for all $s,s' \in \calScom_k$,   $w_k(s) - w_k(s') =\wt{h}_k(s) - \wt{h}_k(s') \leq \rmaxbound D_c$.
We can now focus on the reverse inequality. In this case \tucrl suffers the maximum per-step regret $\rmaxbound$ but the number of times this event happen is ``small'' (see App.~\ref{sec:poorly.visited.states} for details):
\begin{lemma}\label{lem:sum.bad.states}
 For any $T \geq 1$ and any sequence of states and actions $\lbrace s_1, a_1, \dots \dots s_T, a_T \rbrace$ we have: 
\begin{align*}
        \sum_{k=1}^{m}\sum_{s,a}\nu_k(s,a)\mathbbm{1}\lbrace N_k^{\pm}(s,a)\leq\sqrt{\sfrac{t_k}{SA}}\rbrace 
        &\leq
        \sum_{t=1}^{T}\mathbbm{1}\left\{ \max \lbrace 1, N_{k_t}(s_t,a_t)-1 \rbrace\leq \sqrt{\sfrac{t}{SA}} \right\} \\ % := D_T
        &\leq 2\sqrt{SAT} + 2SA
\end{align*}
%and $D_T \leq 2\sqrt{SAT} +2SA$.
\end{lemma}

